Does Reasoning Improve Psychological Depth in Large Language Models? It Depends on Who's Judging

LLM-as-a-Judge evaluators are increasingly used to score open-ended generation, yet a judge's correlation with human ratings on its development set may not guarantee valid measurement when outputs are closely matched and human preferences are subjective. We study this failure mode through psychological depth in short stories. Seven human readers and an LLM-judge ensemble selected on the original scalar Psychological Depth Scale dataset ($\rho = 0.646$) evaluated 60 blinded, prompt-matched story pairs from GPT-5 vs.\ GPT-4o and DeepSeek-R1 vs.\ DeepSeek-V3. Human preferences showed no universal reasoning advantage: GPT-5 was modestly preferred over GPT-4o (60.0--62.9\%), whereas DeepSeek-R1 trailed V3 (42.9\%), and inter-reader agreement was near chance (Krippendorff's $\alpha = 0.070$), with within-reader consistency and recurring weighting patterns suggesting structured heterogeneity rather than random responding. The judge, by contrast, favored reasoning outputs in 89.0\% of dimension-level comparisons and 59 of 60 pairs on aggregate PDS, uniformly across all five evaluator configurations, and its scores were associated with surface features such as sentence length and lexical diversity. These results suggest that development-set performance is insufficient evidence for deployment validity on a shifted distribution, and that point-estimate judges can obscure the heterogeneity in subjective human evaluation.

==> Neurips_workshop/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> content/00_abstract.tex <==
\begin{abstract}
Reasoning-enhanced large language models (LLMs) are assumed to excel across all complex generative tasks, but this remains untested in creative writing. We evaluate reasoning versus non-reasoning frontier LLMs (GPT-5 vs.\ GPT-4o; DeepSeek-R1 vs.\ DeepSeek-V3) on the psychological depth of generated short stories. Using 60 blinded pairwise comparisons, we contrast judgments from seven human annotators against a rigorously validated LLM-as-a-Judge ensemble. Humans exhibited only a marginal preference for reasoning models (55.2\%) with near-chance agreement (Krippendorff's $\alpha = 0.070$). This indicates frontier models have entered a ``low separation zone'' where subjective variance entirely dominates evaluation. Conversely, the automated judge demonstrated a massive, systematic bias, preferring reasoning models in 98.3\% of cases. These findings expose critical flaws in both human and automated evaluation paradigms for frontier creative generation.
\end{abstract}

==> content/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

The rapid scaling of test-time compute in large language models (LLMs) has produced a new generation of \emph{reasoning-enhanced} systems, including GPT-5 \citep{singh2025openaigpt5card} and DeepSeek-R1 \citep{Guo_2025}. These models achieve state-of-the-art results on mathematical and logical benchmarks through extended chain-of-thought inference \citep{openai-o1,snell2024scaling}. This success has sparked a natural but largely untested assumption: that enhanced reasoning capabilities will universally translate to superior performance in complex, open-ended domains, such as creative writing. 

To test this assumption, we investigate whether explicit reasoning actually improves the \emph{psychological depth} of LLM-generated fiction. Psychological depth---encompassing dimensions such as authenticity, empathy, engagement, emotion provocation, and narrative complexity---was recently established as a multidimensional metric for creative generation quality by \citet{harelcanada2024measuringpsychologicaldepthlanguage}. 

However, attempting to systematically measure these highly subjective, nuanced textual properties at the frontier exposes a critical evaluation gap. Standard evaluation protocols heavily rely on aggregate human preference \citep{ouyang2022training, bai2022training} or automated LLM-as-a-Judge systems \citep{zheng2023judgingllmasajudgemtbenchchatbot, dubois2024alpacaeval}. Yet, it remains entirely unclear if these tools are equipped to capture the subtle stylistic and emotional differences between frontier models \citep{clark-etal-2021-thats, chakrabarty2024art, kirk2024prism}.

To probe both the reasoning models' true capabilities and the limits of our current evaluation paradigms, we construct a dual-evaluation study. We curate a dataset of 60 blinded pairwise story comparisons across three model matchups: GPT-5 versus GPT-4o (under both \emph{auto} and \emph{high} reasoning budgets), and DeepSeek-R1 versus DeepSeek-V3. 

We capture highly detailed preference judgments across all five Psychological Depth Scale (PDS) dimensions using a cohort of seven human annotators, contrasted against parallel assessments from a rigorously validated ensemble LLM-as-a-Judge. This design perfectly isolates the boundaries of our current metrics, revealing two major findings:

\paragraph{Finding 1: Human Heterogeneity and the Evaluation Plateau.}
Although reasoning models manage to gain a marginal aggregate preference over their standard counterparts ($55.2\%$), this slight statistical advantage is trivial. The far more significant finding is the extreme divergence among individual annotators: inter-annotator agreement plummeted to barely above chance (Krippendorff's $\alpha = 0.070$). Instead of demonstrating a clear consensus on the superiority of reasoning models, human evaluators behaved wildly differently from each other. This indicates that human preference metrics for frontier models have reached an \textbf{evaluation plateau}. Generation quality has crossed a threshold where objective flaws are rare and idiosyncratic human subjectivity entirely dictates preference. 

\paragraph{Finding 2: Systematic LLM Judge Bias.}
In stark contrast to the heterogeneous and subjective spread of human evaluators, the automatic LLM judge exhibits a rigid and massive bias. The auto-evaluator selected the reasoning model in $98.3\%$ of preference comparisons, assigning significantly higher Likert scores across the board. This rigid preference directly contradicts human readers; in the case of the DeepSeek evaluations, human-judge agreement dropped to exactly $50.0\%$, equivalent to a random coin toss.

These findings carry immediate practical implications: \emph{(i)} LLM-as-a-Judge evaluators possess systematic biases toward reasoning artifacts and cannot be trusted as proxies for human preference on nuanced creative tasks without rigorous auditing, and \emph{(ii)} the field must transition toward evaluation frameworks that characterize the \emph{distribution} of human preferences rather than collapsing them into misleading aggregate win-rates.

==> content/02_related_works.tex <==
\section{Related Work}

\subsection{Evaluating Creativity and Psychological Depth in LLMs}
Evaluating creative text in NLP remains challenging. While \citet{gomez-rodriguez-williams-2023-confederacy} provide comprehensive LLM assessments for creative writing, \citet{chakrabarty2024art} question whether LLMs genuinely exhibit creativity or merely mimic surface patterns. Automated benchmarks like the Torrance Test of Creative Writing (TTCW) \cite{chakrabarty2024art} measure fluency, flexibility, originality, and elaboration. Traditional metrics such as perplexity often reflect fluency rather than novelty \cite{lu2025rethinking}, and LLM-as-a-Judge approaches can be unstable or biased under minor prompt changes. Alignment strategies may inadvertently reduce creative "uncertainty" and "surprise", producing formulaic outputs compared to professional human writing.

Beyond creativity, assessing the psychological impact of LLM-generated narratives has gained attention. Most relevant to our work, \citet{harelcanada2024measuringpsychologicaldepthlanguage} introduce the Psychological Depth Scale (PDS), evaluates an LLM’s capacity to evoke emotion, empathy, and engagement while maintaining narrative complexity and authenticity. Validated with high human consistency (0.72 Krippendorff’s alpha), PDS shows that advanced models like GPT-4 \cite{achiam2023gpt} can produce stories statistically comparable to or surpassing highly-rated human content in empathy and narrative richness.

We extend the PDS framework to pairwise preference evaluation, integrating cognitive-structural and automated metrics to better capture LLMs’ creative and psychological capacities.

\subsection{From Logic to Narrative: The Reasoning Transfer Gap}
Test-time compute scaling has emerged as a powerful paradigm for improving LLM capabilities. OpenAI's o1 \citep{openai-o1} and GPT-5 \citep{singh2025openaigpt5card} apply extended reasoning chains during inference, while DeepSeek-R1 \citep{Guo_2025} achieves similar effects through reinforcement learning. \citet{snell2024scaling} demonstrate that scaling inference-time compute can outperform parameter scaling on reasoning benchmarks. This success has sparked a natural but largely untested assumption: that enhanced reasoning capabilities will universally translate to superior performance in complex, open-ended domains, such as creative writing. However, whether these gains transfer to subjective generative tasks remains an open question. For instance, DeepSeek-R1 serves as a direct reasoning RL upgrade built upon the DeepSeek-V3 \cite{liu2024deepseek} base model, allowing for the isolation of the reasoning RL phase's impact on narrative quality. Anecdotal concerns and widespread public sentiment suggest a preference for GPT-4o's \cite{hurst2024gpt} conversational style over GPT-5's outputs, raising the possibility that reasoning mechanisms introduce negative stylistic artifacts that harm human interaction and narrative resonance. 

Systematic evaluation on narrative and psychological dimensions is lacking, particularly as frontier models may have entered an "evaluation plateau" where objective flaws are rare and individual human subjectivity dictates preference.


\subsection{LLM-as-a-Judge: From Uniform Alignment to Personalized Evaluation}

While the “LLM-as-a-judge” paradigm \citep{zheng2023judgingllmasajudgemtbenchchatbot} provides a scalable alternative to human annotation, existing frameworks often exhibit systematic misalignment due to inherent biases—such as position, verbosity, and self-enhancement—as well as their reliance on uniform, one-size-fits-all scoring rubrics \citep{li-etal-2025-generation}. A central driver of this misalignment is the fundamentally subjective nature of evaluation \cite{dong-etal-2024-llm}, which depends on user-specific personas \cite{dong-etal-2024-llm} and multi-session contextual preferences \cite{liu-etal-2025-persona}. Consequently, model-centric evaluation heuristics often fail to capture the nuanced, preference-driven dynamics underlying human judgment.

Traditionally, many evaluators adopt Likert scales to assign absolute, pointwise ratings. However, such scales often struggle to capture fine-grained distinctions and are susceptible to calibration inconsistencies across judges. To address these limitations, \citet{liu2024aligning} propose pairwise evaluation, which replaces absolute scoring with uncertainty-aware comparative ranking and better aligns with human judgment. Nevertheless, recent findings indicate that the comparative nature of pairwise evaluation can itself amplify certain biases \cite{jeong-etal-2025-comparative}.

Motivated by these limitations, we further identify a bias toward reasoning-model outputs, highlighting the need for personalized evaluation and bridging the gap between rigid, model-centric metrics and nuanced, preference-driven human judgment.


\subsection{Subjective Disagreement and Annotator Heterogeneity}
Research on disagreement and annotator heterogeneity in LLM evaluation has shifted from treating labeling variance as noise to recognizing it as a meaningful signal of subjective human values and task ambiguity \citep{kirk2024prism, sandri-etal-2023-dont}. Prior work shows that standard alignment methods, such as DPO \cite{rafailov2023direct}, often fail to capture diversity across user groups, resulting in “majority-rule” biases that marginalize minority perspectives. To address this limitation, recent approaches—including pluralistic alignment frameworks \cite{chen2024pal}, distributional reward models \cite{dorka2024quantile}, and subjectivity-aware evaluation metrics \cite{fleisig-etal-2023-majority}—explicitly model systematic differences in how individuals and demographics evaluate content. By incorporating annotator-specific context, these methods move toward representing the inherent diversity of human judgment rather than enforcing a single consensus. In subjective NLP tasks, low inter-annotator agreement should not be interpreted as annotation failure; instead, it often reflects genuine differences in evaluative criteria \citep{clark-etal-2021-thats, sandri-etal-2023-dont}. Building on this perspective, our analysis demonstrates that structured variation in how annotators weight PDS dimensions accounts for a substantial portion of the observed disagreement.


==> content/03_dataset.tex <==
\section{\textsc{PsychDepth Reasoning} Dataset}
% \section{Dataset}
\label{sec:dataset}

We construct the \textsc{PsychDepth Reasoning} dataset, comprising 60 pairwise story comparisons generated from 20 carefully curated premises. 

\paragraph{Premise Selection.}
To elicit psychological depth, we required premises that provide sufficient contextual framing for character development while leaving the narrative direction open. We sourced 15 premises from Reddit's r/WritingPrompts, a highly popular online community known for its thematic diversity and structured, high-concept speculative prompts. To prevent data contamination and ensure the models generated genuinely novel narratives rather than recalling memorized text, we strictly sourced prompts posted \emph{after} the known training data cut-off dates for GPT-5 and DeepSeek-R1. From this temporally filtered pool, we sorted by the highest all-time upvotes to ensure strong baseline quality, manually filtering out a small number of prompts containing inappropriate or overtly explicit content.

To ensure our evaluation was not biased solely toward community-driven or speculative fiction, we sourced the remaining 5 premises from Reedsy, a professional platform for authors that curates traditional, grounded literary prompts. Because Reedsy does not provide public engagement metrics (such as upvotes) to serve as a proxy for premise quality, these 5 prompts were uniformly randomly sampled from their database. This split ensures our dataset rigorously tests the models across a diverse spectrum of creative constraints, from imaginative world-building to conventional, character-driven setups. The complete list of all 20 premises used in our evaluation is provided in Appendix~\ref{app:premises}.

\paragraph{Model Pairings and Motivation.}
Our primary objective is to investigate the effects of reasoning-focused reinforcement learning (RL) on creative generation—a domain far removed from the math and coding benchmarks where these models typically excel. We selected two specific model families to serve as our testbeds, generating stories using an identical zero-shot prompt that instructed the models to write a short story based on the given premise. This produced 60 total evaluation pairs:

\begin{description}
    \item[1. DeepSeek-R1 vs.\ DeepSeek-V3 (20 pairs).] \hfill \\
    DeepSeek-R1 \citep{Guo_2025} garnered immense popularity over the last year for its advanced reasoning capabilities. Crucially for our study, it serves as an ideal controlled variable: R1 is a direct reasoning RL upgrade built upon the DeepSeek-V3 base model. Comparing these two allows us to effectively isolate the impact of the reasoning RL phase on narrative quality and psychological depth.

    \item[2. GPT-5 vs.\ GPT-4o (40 pairs).] \hfill \\
    While GPT-5 \citep{singh2025openaigpt5card} does not represent the same strictly isolated RL upgrade path as DeepSeek, it is arguably the most widely accessible and heavily utilized frontier reasoning model by the general public. Recently, widespread anecdotal sentiment has suggested a public preference for GPT-4o's conversational and creative style over GPT-5's outputs. This motivated us to empirically investigate whether the reasoning RL mechanisms driving GPT-5 introduce negative stylistic artifacts that harm human interaction and narrative resonance. To thoroughly test this, we evaluate GPT-5 against GPT-4o under two distinct reasoning budget setting: \textbf{GPT-5 (auto)} (20 pairs) and \textbf{GPT-5 (high)} (20 pairs).
\end{description}


For all subsequent pairwise evaluations, the generated stories for each premise were presented to both human annotators and the automatic evaluator in a blinded, randomized order to completely eliminate positional bias.

==> content/04_human_study.tex <==
\section{Human Study}
Adapting the framework introduced by \citet{harelcanada2024measuringpsychologicaldepthlanguage}, we designed a blinded, pairwise preference annotation protocol to evaluate psychological depth. The study was reviewed by an Institutional Review Board (IRB) and determined to be exempt.

\paragraph{Participant Recruiting.} 
We recruited undergraduate students from the English and Psychology departments at a large research university using targeted interest application forms. We hypothesized that participants with an aptitude for literary and psychological analysis would provide more valuable, nuanced insights than a random cross-section of the population. From 70 applications, we selected the 7 most promising candidates based on their English proficiency, stated interest in the research objectives, and previous experience reviewing short stories. Our goal was to engage informed laypeople with relevant backgrounds, bridging the gap between typical crowdsourced workers and expert professionals.

\paragraph{Evaluation Protocol.} 
We conducted comprehensive online onboarding sessions to introduce the PDS and outline the annotation task. During these meetings, we guided the annotators through the precise definitions of the five PDS metrics and provided training on our custom Label Studio annotation interface, answering any questions to help them calibrate their understanding. After confirming task comprehension, participants were instructed to complete the annotations independently and remotely within seven days. 

To mitigate ordering bias, our pairwise comparison interface presented the two generated stories for each of the 60 pairs side-by-side in a randomized (shuffled) order, with the PDS rubric displayed persistently at the top of the page as a reference. The evaluation criteria required participants to: (1) read the stories thoroughly; (2) select their pairwise preference for each of the five PDS dimensions (authenticity, empathy, engagement, emotion provocation, and narrative complexity); (3) select an overall holistic preference; and (4) provide free-text justifications explaining their selections. Participants were compensated \$100 each for their contributions. In total, this study produced a rich dataset comprising $7 \times 60 \times 6 = 2{,}520$ pairwise preference judgments, alongside extensive qualitative comments.

==> content/05_LLM_judge.tex <==
\section{Automatic Evaluator}
\label{sec:auto}

\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcccccc}
\toprule
\textbf{Evaluator} & \textbf{AUT} & \textbf{PROV} & \textbf{EMP} & \textbf{ENG} & \textbf{NCOM} & \textbf{Overall} \\
\midrule
\textbf{Llama 3.1 70B demo=7}   & 0.576 & 0.674 & 0.637 & 0.507 & 0.637 & \textbf{0.606} \\
\textbf{Llama 3.1 70B demo=5}   & \textbf{0.588} & 0.655 & 0.596 & 0.450 & 0.575 & 0.573 \\
\textbf{Llama 3.1 70B demo=10}  & 0.561 & \textbf{0.702} & 0.671 & 0.387 & 0.568 & 0.578 \\
\textbf{Llama 3.3 70B demo=10}  & 0.580 & 0.676 & \textbf{0.702} & 0.407 & 0.550 & 0.583 \\
\textbf{Qwen3.5 demo=7}      & 0.511 & 0.663 & 0.602 & \textbf{0.564} & 0.496 & 0.567 \\
\textbf{Llama 3.1 70B CoT demo=10} & 0.499 & 0.627 & 0.658 & 0.356 & \textbf{0.664} & 0.561 \\
\midrule
\textbf{Ensemble} & \textbf{0.588} & \textbf{0.702} & \textbf{0.702} & \textbf{0.564} & \textbf{0.664} & \textbf{0.646} \\
\bottomrule
\end{tabular}
\caption{Evaluator Spearman correlation ($\rho$) performance across models and prompting strategies. The bolded values in the upper section highlight the optimal configuration for each specific dimension, which are then combined to form the final routing Ensemble.}
\label{tab:evaluator_comparison_transposed}
\end{table*}

To compare automatic and human judgments, we construct an LLM-as-a-Judge pipeline that extends the zero-shot evaluation framework of \citet{harelcanada2024measuringpsychologicaldepthlanguage} to a controlled few-shot paradigm.

\subsection{Evaluator Construction}

Our pipeline uses DSPy \citep{dspy} to enforce structured output control, ensuring that LLM judges consistently return 1-to-5 Likert scale ratings.
We retain the Mixture-of-Personas (MoP) prompting strategy from the foundational PDS study \citep{harelcanada2024measuringpsychologicaldepthlanguage}, which primes evaluators with distinct analytical perspectives (e.g., literary critic, psychologist) to improve assessment of multifaceted subjective criteria \citep{salewski2023context}.

To construct in-context demonstrations, we use the original 97-story dataset and its five-evaluator human annotations from \citet{harelcanada2024measuringpsychologicaldepthlanguage}.
We partition this data into a 20\% demonstration pool and an 80\% validation split, then apply $k$-means clustering on the PDS score vectors to select semantically representative examples as few-shot demonstrations, rather than relying on random sampling \citep{su2022selective}.

\subsection{Validation}
\label{sec:validation}

We validate evaluator performance on the 80\% held-out split, measuring Spearman correlation ($\rho$) with average human ratings. We experiment across multiple base models, specifically variants of the Llama 3 family \citep{grattafiori2024llama3herdmodels} (Llama~3.1~70B, Llama~3.3~70B) and the Qwen family \citep{qwen35blog} (Qwen3.5-397B-A17B). We vary demonstration counts ($k \in \{5, 7, 10\}$) and test the inclusion of Chain-of-Thought (CoT) prompting \citep{wei2022chain}. The full performance breakdown across all five PDS dimensions is presented in Table~\ref{tab:evaluator_comparison_transposed}.

The best single-model configuration---Llama~3.1~70B with 7 demonstrations---achieves the highest overall average correlation ($\rho = 0.606$). However, Table~\ref{tab:evaluator_comparison_transposed} clearly reveals that psychological depth is a heterogeneous construct; no single model or prompting strategy optimally captures every dimension. For instance, evaluating structural elements like narrative complexity (NCOM) benefits heavily from the explicit reasoning steps provided by CoT ($\rho = 0.664$). In contrast, evaluating holistic or affective qualities achieves higher alignment through standard few-shot prompting across different configurations, such as Qwen3.5 for engagement ($\rho = 0.564$) or Llama~3.3~70B for empathy ($\rho = 0.702$). This variance demonstrates that different dimensions of narrative quality require distinct evaluative mechanisms.

\subsection{Ensemble Evaluator}

To maximize reliability, we construct a heterogeneous ensemble that capitalizes on the metric-specific strengths identified during validation. We build the ensemble by routing the evaluation of each PDS metric to its independently best-performing model configuration. 

As shown in the final row of Table~\ref{tab:evaluator_comparison_transposed}, this routing strategy yields an ensemble correlation of $\rho = 0.646$. This substantially exceeds the performance of any single-model configuration and represents a major improvement upon the zero-shot approach of \citet{harelcanada2024measuringpsychologicaldepthlanguage} ($\rho \approx 0.51$ with GPT-4o), providing a highly robust automated judge for our pairwise experiments.

\subsection{Pairwise Inference Protocol}
\label{sec:pairwise_inference}

While our experimental setup requires pairwise preference selections, our pipeline is deliberately designed to predict 1-to-5 continuous Likert ratings. We chose a rating-based evaluator because our foundational study provides the highest-quality supervision available for this construct: dimension-aligned, scalar PDS annotations with strong inter-annotator agreement. 

This formulation provides two critical advantages over a directly pairwise-trained evaluator: (1) dimension-aligned supervision for few-shot prompt calibration, and (2) a quantitative held-out benchmark for validating human-evaluator alignment prior to deployment, as demonstrated in Section~\ref{sec:validation}.

To align this robust scalar evaluator with our pairwise experimental design, we convert the Likert outputs into pairwise comparisons at inference time. For each of the 60 story pairs, the ensemble evaluates Story A and Story B independently. We then compare the predicted PDS scores, selecting the higher-scoring story as the preference, and defaulting to a tie if the scores are identical.

==> content/06_results_analysis.tex <==
\section{Results}
\label{sec:results}


\begin{table}[ht]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Pair} & \textbf{Pref.} & \textbf{All 6} \\
\midrule
GPT-5 (auto) vs.\ 4o & 60.0\% & 61.4\% \\
GPT-5 (high) vs.\ 4o & 62.9\% & 60.8\% \\
DeepSeek-R1 vs.\ V3 & 42.9\% & 50.5\% \\
\midrule
\textbf{Overall} & \textbf{55.2\%} & \textbf{57.6\%} \\
\bottomrule
\end{tabular}
\caption{Human preference rate for the reasoning model.
\textbf{Pref.}\ = overall preference metric only; \textbf{All~6} = pooled across all six evaluation dimensions (5 PDS + preference). Rates represent the proportion of annotator votes favoring the reasoning model.}
\label{tab:human_pref}
\end{table}

\begin{table}[ht]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Metric} & \textbf{Fleiss' $\kappa$} & \textbf{Kripp.\ $\alpha$} & \textbf{Raw} \\
\midrule
Authenticity & 0.035 & 0.037 & 52.5\% \\
Emotion Prov. & 0.080 & 0.082 & 54.1\% \\
Empathy & \textbf{0.182} & \textbf{0.185} & \textbf{59.1\%} \\
Engagement & 0.059 & 0.061 & 53.3\% \\
Narr.\ Complexity & 0.016 & 0.018 & 52.1\% \\
Preference & 0.035 & 0.038 & 51.9\% \\
\midrule
\textbf{Average} & \textbf{0.068} & \textbf{0.070} & \textbf{53.8\%} \\
\bottomrule
\end{tabular}
\caption{Inter-annotator agreement across 60 pairs and 7 annotators. Fleiss' $\kappa$ \citep{fleiss1971measuring} and Krippendorff's $\alpha$ \citep{krippendorff2011computing} are computed on nominal-scale pairwise selections. Raw = average pairwise agreement rate.}
\label{tab:iaa}
\end{table}

\begin{table}[ht]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Pair} & \textbf{Pref.} & \textbf{All 6} \\
\midrule
GPT-5 (auto) vs.\ 4o & 100.0\% & 96.7\% \\
GPT-5 (high) vs.\ 4o & 100.0\% & 90.8\% \\
DeepSeek-R1 vs.\ V3 & 95.0\% & 80.0\% \\
\midrule
\textbf{Overall} & \textbf{98.3\%} & \textbf{89.2\%} \\
\bottomrule
\end{tabular}
\caption{Automatic evaluator preference rate for the reasoning model. Format follows Table~\ref{tab:human_pref}.}
\label{tab:auto_pref}
\end{table}

% \begin{table}[ht]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Metric} & \textbf{All} & \textbf{DS} & \textbf{GPT} \\
% \midrule
% Authenticity & 50.0\% & 40.0\% & 55.0\% \\
% Emotion Prov. & 76.7\% & 60.0\% & 85.0\% \\
% Empathy & 78.3\% & 75.0\% & 80.0\% \\
% Engagement & 63.3\% & 40.0\% & 75.0\% \\
% Narr.\ Complexity & 60.0\% & 55.0\% & 62.5\% \\
% Preference & 56.7\% & 30.0\% & 70.0\% \\
% \midrule
% \textbf{Average} & \textbf{64.2\%} & \textbf{50.0\%} & \textbf{71.3\%} \\
% \bottomrule
% \end{tabular}
% \caption{Agreement between the auto-evaluator and human majority vote. \textbf{DS} = DeepSeek-R1 vs.\ V3; \textbf{GPT} = GPT-5 vs.\ GPT-4o (both reasoning budgets pooled).}
% \label{tab:alignment}
% \end{table}


\begin{table}[ht]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Pair} & \textbf{$\Delta$ Score} & \textbf{Cohen's $d$} & \textbf{$p$-value} \\
\midrule
GPT-5 (auto) & $+0.518$ & 1.143 & $<\!0.001$ \\
GPT-5 (high) & $+0.500$ & 1.121 & $<\!0.001$ \\
DeepSeek & $+0.214$ & 0.681 & $<\!0.001$ \\
\midrule
\textbf{Overall} & $\mathbf{+0.411}$ & $\mathbf{0.952}$ & $\mathbf{<\!0.001}$ \\
\bottomrule
\end{tabular}
\caption{Auto-evaluator bias toward reasoning models, measured as the mean Likert score difference (reasoning $-$ non-reasoning) pooled across all five PDS metrics. Cohen's $d$ computed on paired differences; $p$-values from paired $t$-tests.}
\label{tab:bias}
\end{table}

\begin{table*}[t]
\centering
\caption{Differences between Reasoning (R) and Non-Reasoning (NR) models across psychological depth metrics using the
Ensemble Evaluator.}
\label{tab:psych_depth_comparison}
\begin{tabular}{lcccccc}
\toprule
\textbf{Metric} & \textbf{R Avg} & \textbf{NR Avg} & \textbf{Mean Diff} & \textbf{95\% CI} & \textbf{Cohen's $d$} &
\textbf{$p$-value} \\
\midrule
Authenticity          & 4.817 & 4.555 & +0.262 & {[}+0.206, +0.318{]} & 1.205 & $<\!0.001$ \\
Emotion Provoking     & 4.817 & 4.148 & +0.669 & {[}+0.536, +0.802{]} & 1.299 & $<\!0.001$ \\
Empathy               & 4.864 & 4.643 & +0.221 & {[}+0.152, +0.290{]} & 0.824 & $<\!0.001$ \\
Engagement            & 4.875 & 4.169 & +0.707 & {[}+0.579, +0.835{]} & 1.425 & $<\!0.001$ \\
Narrative Complexity  & 4.608 & 4.412 & +0.196 & {[}+0.138, +0.254{]} & 0.870 & $<\!0.001$ \\
\midrule
Overall               & 4.796 & 4.385 & +0.411 & {[}+0.362, +0.460{]} & 0.952 & $<\!0.001$ \\
\bottomrule
\end{tabular}
\end{table*}


Our experimental design was strictly constructed to yield high-signal evaluations: we utilized a validated multidimensional rubric (PDS), a rigorously calibrated LLM-as-a-Judge, and a screened human annotator pool. However, the resulting data reveals a severe misalignment between human subjective reception and automated assessment, exposing critical failure modes in frontier model evaluation.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figs/reasoning_preference_deepseek_gpt_auto.png}
\caption{Preference rates for reasoning models across 7 individual human annotators, the human average, and the automated LLM judge (aggregated over 40 pairs). The stark patchwork of variance among Annotators 1--7 illustrates the ``evaluation plateau'' of human subjectivity, while the far-right Auto column exposes the rigid, systematic bias of the LLM evaluator.}
\label{fig:annotator_heatmap}
\end{figure*}

\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{figs/fig_auto_majority_agreement_combined.png}
\caption{Agreement rates between the automated LLM judge and human majority vote across different model pairings. The dashed vertical line represents 50\% (random chance). The DeepSeek-R1 vs.\ V3 pairing exposes severe misalignment, with the LLM judge agreeing with human preference only 30\% of the time.}
\label{fig:alignment}
\end{figure*}

% \subsection{Human Heterogeneity and the Evaluation Plateau}
% \label{sec:human_results}

% We first examine the human preference rates (Table~\ref{tab:human_pref}). Across all 60 pairs, the aggregate human preference for the reasoning models over their standard counterparts is a marginal $55.2\%$. 

% Crucially, this tepid aggregate win-rate is not indicative of models performing equally well in the eyes of the readers; rather, it masks a complete collapse in reader consensus. As shown in Table~\ref{tab:iaa}, inter-annotator agreement plummeted to effectively random noise (average Krippendorff's $\alpha = 0.070$, Fleiss' $\kappa = 0.068$). Even the most agreed-upon dimension, Empathy ($\alpha = 0.185$), fails to reach the minimum threshold for ``fair agreement,'' while dimensions like Authenticity ($\alpha = 0.037$) and Narrative Complexity ($\alpha = 0.018$) exhibit no reliable consensus whatsoever.



% This is a profound deviation from the foundational PDS study \citep{harelcanada2024measuringpsychologicaldepthlanguage}, which reported strong inter-annotator agreement ($\alpha \approx 0.72$) using an identical rubric on older models. This dramatic drop in our pairwise setting suggests that frontier generation quality has crossed an \textbf{evaluation plateau}. The objective flaws that previously drove human consensus (e.g., grammatical errors, severe hallucinations, disjointed plots) have been solved. At this frontier, subjective variance and idiosyncratic reader taste entirely dominate the assessment of creative writing. 

% Furthermore, reasoning RL does not universally align with human literary taste. While humans showed a slight preference for GPT-5 over GPT-4o, they actively \emph{dispreferred} DeepSeek-R1 compared to its base model, DeepSeek-V3 ($42.9\%$). 

\subsection{Human Heterogeneity and the Evaluation Plateau}
\label{sec:human_results}

We first examine the human preference rates (Table~\ref{tab:human_pref}). Across all 60 pairs, the aggregate human preference for the reasoning models over their standard counterparts is a marginal $55.2\%$. 

Crucially, this tepid aggregate win-rate is not indicative of a mild consensus where all readers found the models to be of roughly equal quality. Instead, it masks a deep polarization in reader reception. While there are relatively consistent signals favoring reasoning models on specific affective dimensions---most notably \emph{emotion provocation} (where the human average peaks at $66.1\%$ in the GPT pairings) and \emph{empathy}---we cannot confidently conclude a universal preference for reasoning models because a true ``aggregated opinion'' simply does not exist.

This profound divergence is visually stark in Figure~\ref{fig:annotator_heatmap}. Across the individual human columns (Ann 1 to Ann 7), we observe a chaotic patchwork of subjective preference. The variance between individual annotators is extreme: Annotator 7 predominantly favors the reasoning models, preferring them $70.0\%$ to $80.0\%$ of the time across nearly all dimensions. In sharp contrast, Annotator 1 actively penalizes the reasoning models, exhibiting a strong preference for the non-reasoning baseline models (e.g., favoring the reasoning model only $27.5\%$ of the time for engagement, and $32.5\%$ for overall preference). 

Because of these extreme subjective splits, inter-annotator agreement plummeted to effectively random noise (Table~\ref{tab:iaa}), averaging Krippendorff's $\alpha = 0.070$. Even the most agreed-upon dimension, Empathy ($\alpha = 0.185$), fails to reach the minimum threshold for ``fair agreement.'' 

This is a profound deviation from the foundational PDS study \citep{harelcanada2024measuringpsychologicaldepthlanguage}, which reported strong inter-annotator agreement ($\alpha \approx 0.72$) using an identical rubric on older models. This dramatic drop in our pairwise setting suggests that frontier generation quality has crossed an \textbf{evaluation plateau}. When one reader strongly prefers a story and another strongly rejects it, collapsing their opposing views into a $50\%$ ``tie'' or a $55\%$ ``marginal win'' is statistically misleading. It proves that at the frontier of generation quality, the ``average reader'' is a mathematical illusion; idiosyncratic subjective variance entirely dictates narrative preference.

\subsection{The Illusion of Consensus: Automated Evaluator Bias}
\label{sec:auto_results}

If we were to evaluate these models relying solely on our validated LLM-as-a-Judge ensemble, which is a standard practice in contemporary NLP, we would arrive at a drastically different and highly misleading conclusion. 

As shown in Table~\ref{tab:auto_pref}, the automatic evaluator exhibits a rigid, overwhelming preference for reasoning models, selecting them in $95.0\%$ of overall preference matchups. For the GPT-5 pairings, the auto-evaluator assigned a perfect $100\%$ preference rate, entirely blind to the $37$--$40\%$ of human readers who preferred GPT-4o's stylistic output. 

This creates a severe human-judge misalignment, vividly illustrated in Figure~\ref{fig:alignment}. This failure is most glaringly exposed in the DeepSeek-R1 vs.\ V3 matchup. While humans preferred the non-reasoning V3 model, the LLM judge heavily favored R1 ($95.0\%$). Consequently, as shown by the dashed $50\%$ chance line in Figure~\ref{fig:alignment}, the automated judge frequently fails to exceed random chance in this pairing. Most damningly, the human-judge agreement rate on overall preference plummets to just $30.0\%$, meaning the LLM judge is actively diametrically opposed to human consensus. While alignment slightly recovers in the GPT-5 pairings (where both humans and the judge trended toward the reasoning model), the underlying bias remains clear.

We quantify this systemic misalignment across model families in Table~\ref{tab:bias}. The evaluator assigns reasoning models a massive score advantage (Cohen's $d = 0.952$, $p < 0.001$) \citep{cohen1988statistical}. This bias is most extreme for GPT-5 ($d = 1.143$ for auto, $d = 1.121$ for high) and attenuated but still highly significant for DeepSeek ($d = 0.681$).

Furthermore, breaking down this bias by psychological dimension (Table~\ref{tab:psych_depth_comparison}) reveals exactly where the automated judge diverges from human consensus. The LLM judge artificially inflates the scores of reasoning models most severely on Engagement ($d = 1.425$) and Emotion Provoking ($d = 1.299$). This suggests that the evaluator is highly sensitive to latent stylistic artifacts produced during the reasoning generation phase, incorrectly conflating these features with genuine emotional resonance and narrative captivation—qualities that human readers did not reciprocally reward. Ultimately, this creates a massive false positive for narrative quality.
\section{Discussion}
\label{sec:discussion}

By isolating the impact of reasoning RL on creative writing through the lens of psychological depth, our results expose a critical dual failure mode in how the NLP community evaluates frontier generative models.

\paragraph{The Failure of Aggregate Human Preference.}
The near-chance inter-annotator agreement demonstrates that at the frontier, human pairwise preference is driven almost entirely by idiosyncratic reader taste rather than universally detectable quality differences. Consequently, collapsing these highly divergent human behaviors into a traditional ``majority vote'' win-rate actively obscures the reality of human preference. We cannot rely on aggregate preference to evaluate subjective textual properties when the "average reader" no longer exists.

\paragraph{Reasoning-Model Preference Bias.}
Our findings extend prior work on LLM self-enhancement bias \citep{10.5555/3737916.3740113} and position bias \citep{wang2024large} to a dangerous new modality: \emph{reasoning-model preference bias}. The automated judge's overwhelming preference for reasoning models, directly contradicting human readers (as seen in the DeepSeek matchup), proves that LLM evaluators are systematically biased toward the distinct stylistic distributions of reasoning models. They conflate whatever latent patterns these models produce with actual literary quality. As reasoning models proliferate, relying on automated LLM-as-a-Judge paradigms to assess subjective, creative generation will yield fundamentally invalid conclusions unless these biases are addressed.

==> content/07_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this study, we investigated whether the enhanced reasoning capabilities of frontier large language models translate into superior psychological depth in creative writing. By benchmarking systems such as GPT-5 and DeepSeek-R1 against their non-reasoning counterparts, we have identified critical challenges for current evaluation methodologies.

Our findings yield two primary insights. First, we characterize the \textbf{Evaluation Plateau}: as frontier models converge toward high linguistic quality, objective narrative flaws become rare, causing evaluation to be dominated by idiosyncratic subjective taste. This shift is evidenced by the near-zero inter-annotator agreement ($\alpha = 0.070$) observed in our human study. These results suggest that for open-ended creative tasks, collapsing human preference into a single aggregate win-rate is insufficient; instead, evaluation frameworks should account for the \textit{distribution} of human preferences across diverse reader profiles.

Second, our results expose a systematic \textbf{reasoning-model preference bias} in automated evaluators. We demonstrated that even an ensemble judge, which was previously validated and proven effective on earlier benchmarks, exhibited a rigid preference for reasoning models (98.3\%) that was not shared by human annotators. This misalignment suggests that LLM-as-a-Judge systems are highly sensitive to stylistic artifacts inherent in reasoning-heavy generations, incorrectly conflating these features with narrative quality.

In summary, our study indicates that increased test-time compute does not yield a universal improvement in the affective and psychological dimensions of storytelling. Furthermore, as reasoning models continue to proliferate, relying solely on automated metrics for subjective tasks poses a significant risk of misalignment. We argue that maintaining human-centric oversight remains essential to ensure that generative models align with human resonance rather than internal model biases.

==> content/08_limitation.tex <==
\section{Limitations}
\label{sec:limitations}

Despite the robust experimental framework and the use of a calibrated ensemble evaluator, our study has several limitations that provide context for our findings.

\paragraph{The "Evaluation Plateau" and Subjective Variance.}
As evidenced by the near-zero inter-annotator agreement (Table~\ref{tab:iaa}), our human evaluation encountered an \textbf{evaluation plateau}. Due to the lack of free-text justifications from annotators, we cannot definitively attribute the divergent preferences seen in Figure~\ref{fig:annotator_heatmap} to specific literary elements. We cannot discern, for instance, whether Annotator 1 penalized DeepSeek-R1 for its specific stylistic "artifacts" or if Annotator 7 rewarded GPT-5 for its structural complexity. Future work should incorporate qualitative feedback to decode the "black box" of human subjective reception at the frontier.

\paragraph{Annotation Quality and Signal-to-Noise Ratio.}
While we adopted recruitment protocols from prior studies that yielded clear preference signals, the low Fleiss' $\kappa$ (0.068) in our pairwise setup suggests that the signal-to-noise ratio in creative writing annotation is decreasing as models converge in quality. Although we implemented standard quality controls, more rigorous attention checks or "gold-standard" narrative filters might be necessary to distinguish between genuine subjective disagreement and annotation noise caused by the high cognitive load of comparing two high-quality stories.

\paragraph{Scope of Narrative Premises.}
Our study utilized premises from \textit{Reddit} and \textit{Reedsy}, which are primarily tailored for short-form, prompt-driven creative writing. It is possible that the "reasoning dividend"—the benefit of extensive CoT for narrative depth—only fully manifests in long-form content (e.g., multi-chapter novels) or highly constrained scenarios (e.g., hard science fiction) that were not captured in our current dataset. Expanding the premise pool to include these complex domains is essential to determine if our observed "reasoning-model preference bias" in automated judges persists across all literary genres.

\paragraph{Opaqueness of Automated Evaluator Bias.}
While Table~\ref{tab:bias} and Table~\ref{tab:psych_depth_comparison} clearly quantify a massive, systemic bias in LLM judges toward reasoning models ($d=0.952$), we lack a mechanistic explanation for this misalignment. We do not yet know which specific stylistic or structural markers in reasoning-model outputs trigger the automated "inflation" of scores for dimensions like \textit{Engagement} and \textit{Emotion Provocation}. Investigating the linguistic features that LLM judges conflate with narrative quality remains a critical next step for ensuring the validity of LLM-as-a-Judge paradigms.

==> content_v2/00_abstract.tex <==
\begin{abstract}
% Reasoning-enhanced large language models are often assumed to improve complex generative tasks, but this assumption remains underexplored for creative writing. We study this question through the psychological depth of short stories, comparing frontier reasoning and non-reasoning model pairs (GPT-5 vs.\ GPT-4o; DeepSeek-R1 vs.\ DeepSeek-V3) using 60 blinded pairwise comparisons rated by seven human annotators and an ensemble LLM-as-a-Judge. Human preferences do not support a single global conclusion: while GPT-5 is slightly preferred over GPT-4o (60–63\%), DeepSeek-R1 falls behind DeepSeek-V3 (42.9\%). Although inter-annotator agreement is low (Krippendorff's $\alpha = 0.070$), multiple quality checks suggest that this reflects genuine evaluative subjectivity, possibly driven by differing weighting schemes over psychological-depth dimensions, rather than annotation failure. By contrast, the automatic evaluator prefers the reasoning model 98.3\% of the time, producing a much more uniform pro-reasoning signal than the human cohort. These findings suggest that reasoning enhancement does not have a universal effect on perceived creative quality, that human disagreement constitutes a key signal of irreducible subjectivity in evaluation, and that LLM-as-a-Judge evaluators should be used cautiously for nuanced creative-generation tasks.
Benchmark gains from reasoning-enhanced large language models encourage the assumption that these models should broadly perform better on complex generative tasks, but this remains underexplored in open-ended, creative domains shaped by nuances of reader experience. We tested this assumption through the lens of psychological depth in short stories. We compared frontier reasoning/non-reasoning model pairings (GPT-5 vs. GPT-4o and DeepSeek-R1 vs. DeepSeek-V3) through 60 blinded pairwise evaluations in which seven human annotators and an ensemble LLM-as-a-Judge rated prompt-matched story outputs. Our results showed no universal reasoning advantage in human evaluations: GPT-5 was slightly preferred over GPT-4o under both "auto" (60.0\%) and "high" (62.9\%) reasoning effort settings, whereas DeepSeek-R1 fell behind DeepSeek-V3 (42.9\%). Although this pattern was marked by low inter-annotator agreement (Krippendorff's $\alpha = 0.070$), our annotation-quality checks suggested genuine evaluative subjectivity, plausibly reflecting distinct annotator decision schemes rather than annotation failure. In contrast to the human evaluations, the LLM-as-a-Judge evaluator showed a far more uniform pro-reasoning signal: 100\% in the GPT comparisons and 95.0\% in the DeepSeek comparison. These findings suggest that reasoning enhancement does not have a universal effect on perceived creative quality, that human disagreement can itself mark irreducible subjectivity in evaluation, and that LLM-as-a-Judge evaluators can obscure this subjectivity in nuanced creative-generation tasks.

\end{abstract}


==> content_v2/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}


Reasoning-enhanced language models are routinely evaluated on mathematical, coding, and factual benchmarks \citep{openai-o1,snell2024scaling, chen2026learning, li202512surveyreasoning, zeng2025thinkingloudreasoningmodels,yu2025benchmarking, 10.1145/3774896}. Models such as GPT-5 and DeepSeek-R1 undergo post-training aimed at strengthening deliberative reasoning, often through reinforcement learning or related reasoning-oriented methods \citep{singh2025openaigpt5card, Guo_2025}. However, much less is known about how such post-training affects creative generation. In particular, performance gains on standard benchmarks invite the assumption that the capabilities behind these gains should also generalize to complex, open-ended tasks such as fiction writing, though this has yet to be investigated directly. 

We investigated this question through the lens of \emph{psychological depth} in short stories. We constructed 60 blinded pairwise story comparisons across three frontier model matchups, namely GPT-5 versus GPT-4o under two reasoning effort settings and DeepSeek-R1 versus DeepSeek-V3. To evaluate these pairs, we used the Psychological Depth Scale (PDS) \citep{harelcanada2024measuringpsychologicaldepthlanguage}, which measures authenticity, empathy, engagement, emotion provocation, and narrative complexity. Each story pair was evaluated by seven human annotators and an LLM-as-a-Judge ensemble. We also collected an overall preference to examine how preferences on individual PDS dimensions relate to readers’ overall judgments. 
% in fictional stories. An \emph{overall preference} rating is also collected to examine how judgments on the individual dimensions relate to overall preference. Concretely, we construct 60 blinded pairwise story comparisons spanning three frontier model matchups, namely GPT-5 versus GPT-4o under two reasoning budgets and DeepSeek-R1 versus DeepSeek-V3, and evaluate them with seven human annotators together with a validated ensemble LLM-as-a-Judge. This setup allows us to study not only whether reasoning-enhanced models are preferred, but also whether such preferences hold across model families and readers.

This setup allowed us to test not only whether reasoning-enhanced large language models are preferred, but also whether such preferences hold across model families and readers. More specifically, we asked three questions: \textbf{RQ1.} Do humans prefer reasoning-enhanced LLMs over their non-reasoning counterparts on storywriting tasks? \textbf{RQ2.} Are these preferences consistent across annotators and psychological-depth dimensions? \textbf{RQ3.} Do LLM-as-Judge evaluators recover the same preference patterns as human annotators?

Taken together, our findings suggest a more heterogeneous picture than standard benchmark gains alone would lead one to expect. In comparisons evaluated by human annotators, GPT-5 was preferred over GPT-4o, whereas DeepSeek-R1 fell behind DeepSeek-V3. This contrasts with earlier PDS evaluations, where quality gaps between stories were large enough to yield strong annotator consensus; at the frontier, preferences increasingly reflected individual reader subjectivity rather than detectable quality differences. The human evaluations also showed substantial disagreement, and our quality checks suggest that this reflects genuine evaluative subjectivity rather than annotation failure, plausibly because annotators rely on distinct rationales and weight psychological-depth dimensions differently. In contrast, despite being specifically optimized to maximize agreement with human annotations on the original PDS dataset ($\rho$ = 0.646), the LLM-as-a-Judge evaluator remained strongly pro-reasoning across both model families, which may obscure meaningful variation visible in the human results. Figure~\ref{fig:teaser} illustrates this contrast for a representative story pair: human annotators displayed diverse preferences across PDS dimensions, whereas the LLM-as-Judge ensemble collapsed into unanimous agreement.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/plot.png}
    \caption{\textbf{Evaluating psychological depth: human subjectivity vs. LLM consensus.} Evaluation patterns across five psychological dimensions for a representative story pair (Pair 24, GPT-5 vs.\ GPT-4o). (\textbf{Left}) Human annotators displayed diverse preferences, reflecting subjective interpretations. (\textbf{Right}) The LLM-as-a-judge ensemble collapsed this subjectivity into unanimous preference for the reasoning model. %Blue indicates preference for GPT-5; red indicates preference for GPT-4o.
    }
\label{fig:teaser}
\end{figure}

% \paragraph{RQ1. Do humans prefer reasoning-enhanced LLMs over their non-reasoning counterparts on storywriting tasks?}
% Our results are mixed. Human annotators show a slight preference toward the reasoning-enhanced GPT-5 over GPT-4o, while DeepSeek-R1 and DeepSeek-V3 are near tie. The effect of reasoning enhancement on psychological depth is thus not uniform across frontier model families. This contrasts with earlier PDS evaluations, where quality gaps between stories were large enough to yield strong annotator consensus; at the frontier, generation quality has converged to the point where preferences increasingly reflect individual reader subjectivity rather than detectable quality differences.


% \paragraph{RQ2. Are these preferences consistent across annotators and psychological-depth dimensions?}
% Annotator preferences are diverse and do not converge on a single evaluation pattern. The inter-rater agreement is low, reflecting meaningful variations among readers when evaluating story pairs with no substantial quality gap. On the annotator level, preferences on PDS dimensions exhibit varying levels of agreement with the overall preference and have different predictive power in the logistic regression model, suggesting that individual dimensions are weighted differently when forming the overall preference. The agreement and regression analyses revealed similar clusters among the seven annotators, reflecting distinct decision schemes.

% \paragraph{RQ3. Do automatic evaluators recover the same preference patterns as human annotators?}
% Our ensemble LLM-as-judge evaluator was specifically optimized to maximize agreement with human annotations on the original PDS dataset, achieving strong correlation ($\rho$ = 0.646). Despite this, when applied to frontier story pairs, it produces a more uniformly pro-reasoning signal across our 60 story pairs, flattening family-level and annotator-level heterogeneity that remains significant in the human data. Figure~\ref{fig:teaser} illustrates this contrast for a representative story pair: human annotators display diverse preferences across PDS dimensions, while the LLM-as-Judge ensemble collapses into unanimous agreement.

% Taken together, these findings suggest that the relationship between reasoning enhancement and psychological depth is neither a simple gain nor a simple trade-off. Instead, it is heterogeneous across model families and readers, while automatic evaluators may obscure this heterogeneity by producing a stronger and more homogeneous preference signal than the human cohort warrants.
% The findings suggest that the relationship between reasoning enhancement and psychological depth is neither a simple gain nor a trade-off. Instead, it is heterogeneous across model families and readers, while automatic evaluators may obscure this by producing a stronger, more homogeneous preference signal than the human cohort warrants.

Our paper makes three contributions. First, we present a controlled human evaluation of frontier reasoning and non-reasoning models on short-story generation through the lens of psychological depth. Second, we show that annotator disagreement is a meaningful part of the evaluative phenomenon itself, and we relate that disagreement to distinct dimension-weighting schemes across annotators. Third, we show that a validated LLM-as-a-Judge evaluator yields a much more uniformly pro-reasoning pattern than the human evaluations, posing a challenge for nuanced story evaluation and for alignment with human preferences.

==> content_v2/02_Related_Works.tex <==
\section{Related work}
\label{sec:related}

\paragraph{Psychological depth and creativity evaluation.} Evaluating creative text remains a longstanding challenge in NLP \citep{gomez-rodriguez-williams-2023-confederacy}. Traditional metrics such as perplexity often capture fluency rather than the kinds of qualities that matter in literary evaluation \citep{lu2025rethinking}, and recent work has questioned whether LLMs exhibit genuine creativity or merely reproduce familiar surface patterns \citep{chakrabarty2024art}. Most relevant to our study, \citet{harelcanada2024measuringpsychologicaldepthlanguage} introduce the Psychological Depth Scale (PDS), a five-dimensional framework for evaluating authenticity, empathy, engagement, emotion provocation, and narrative complexity in fictional stories, and demonstrate that human annotators achieve moderate agreement (Krippendorff's $\alpha \approx 0.72$) when rating individual stories on a Likert scale. We build on that framework in a more demanding frontier setting, where quality differences between model outputs are narrower and pairwise comparison better fits the task \citep{liu2024aligning}. Importantly, research on annotator disagreement treats variance in subjective annotation not as noise but as a meaningful signal of value pluralism and task ambiguity \citep{clark-etal-2021-thats, sandri-etal-2023-dont, kirk2024prism}. Our analysis extends this perspective by relating disagreement to differences in how annotators weight dimensions of psychological depth.

\paragraph{Reasoning-enhanced LLMs beyond benchmarks.}
Test-time compute scaling has emerged as a powerful paradigm for improving LLM capabilities. OpenAI's o1 \citep{openai-o1} and GPT-5 \citep{singh2025openaigpt5card} apply extended reasoning chains during inference, while DeepSeek-R1 \citep{Guo_2025} achieves similar effects through reinforcement learning. \citet{snell2024scaling} demonstrate that scaling inference-time compute can outperform parameter scaling on reasoning benchmarks. However, whether these gains transfer to subjective generative tasks remains an open question. DeepSeek-R1 is built upon DeepSeek-V3 with an additional reasoning-oriented RL phase \citep{liu2024deepseek}, providing the most direct comparison available for studying how reasoning post-training affects narrative quality. Anecdotal concerns and widespread public sentiment suggest that reasoning-oriented post-training may alter writing style or creativity, but systematic evaluation on narrative and psychological dimensions is lacking.

% \paragraph{LLM-as-a-Judge and Evaluator Misalignment.}
% The LLM-as-a-Judge paradigm \citep{zheng2023judgingllmasajudgemtbenchchatbot} has become ubiquitous for scalable evaluation, yet existing frameworks often exhibit systematic misalignment due to inherent biases, such as position, verbosity, and self-enhancement, as well as their reliance on uniform scoring rubrics \citep{li-etal-2025-generation}. \citet{10.5555/3737916.3740113} show that LLM evaluators favor their own generations. \citet{stureborg2024large} and \citet{wang2024large} document inconsistency and unfairness in LLM-based judgments. \citet{liu2024aligning} advocate for pairwise evaluation to better align with human judgment, though \citet{jeong-etal-2025-comparative} find that pairwise comparisons can themselves amplify certain biases. Most prior work on evaluator bias focuses on factual or instructional tasks; our work extends this to frontier creative generation and identifies a new modality of bias: systematic preference for reasoning-model outputs.

\paragraph{LLM-as-a-Judge evaluation.} The LLM-as-a-Judge paradigm has become a standard tool for scalable assessment \citep{zheng2023judgingllmasajudgemtbenchchatbot}. Prior work suggests that pairwise formats can align well with human judgment \citep{liu2024aligning}, though more recent work shows that pairwise comparison can also amplify evaluator biases \citep{jeong-etal-2025-comparative}. These concerns are especially relevant for our setting, where the evaluation target is subjective and frontier outputs are often close in quality. They also motivate our decision to ground the evaluator in human-validated scalar judgments and derive pairwise preferences post hoc.

% \paragraph{Disagreement and Annotator Heterogeneity.}
% Research on annotator disagreement has shifted from treating labeling variance as noise to recognizing it as a meaningful signal of subjective human values and task ambiguity \citep{kirk2024prism, sandri-etal-2023-dont}.  In subjective NLP tasks, low inter-annotator agreement does not automatically indicate failed annotation; it can instead reflect genuine differences in evaluative priorities \citep{clark-etal-2021-thats, sandri-etal-2023-dont}. Our analysis builds on this perspective, suggesting that variation in how annotators weight PDS dimensions may contribute to the observed disagreement.

% \subsection{Evaluating Creativity and Psychological Depth in LLMs}
% Evaluating creative text in NLP remains challenging. While \citet{gomez-rodriguez-williams-2023-confederacy} provide comprehensive LLM assessments for creative writing, \citet{chakrabarty2024art} question whether LLMs genuinely exhibit creativity or merely mimic surface patterns. Automated benchmarks like the Torrance Test of Creative Writing (TTCW) \cite{chakrabarty2024art} measure fluency, flexibility, originality, and elaboration. Traditional metrics such as perplexity often reflect fluency rather than novelty \cite{lu2025rethinking}, and LLM-as-a-Judge approaches can be unstable or biased under minor prompt changes. Alignment strategies may inadvertently reduce creative "uncertainty" and "surprise", producing formulaic outputs compared to professional human writing.

% Beyond creativity, assessing the psychological impact of LLM-generated narratives has gained attention. Most relevant to our work, \citet{harelcanada2024measuringpsychologicaldepthlanguage} introduce the Psychological Depth Scale (PDS), evaluates an LLM’s capacity to evoke emotion, empathy, and engagement while maintaining narrative complexity and authenticity. Validated with high human consistency (0.72 Krippendorff’s alpha), PDS shows that advanced models like GPT-4 \cite{achiam2023gpt} can produce stories statistically comparable to or surpassing highly-rated human content in empathy and narrative richness.

% We extend the PDS framework to pairwise preference evaluation, using the cognitive-structural dimensions in PDS to better capture LLMs’ creative and psychological capacities.

% \subsection{From Logic to Narrative: The Reasoning Transfer Gap}
% Test-time compute scaling has emerged as a powerful paradigm for improving LLM capabilities. OpenAI's o1 \citep{openai-o1} and GPT-5 \citep{singh2025openaigpt5card} apply extended reasoning chains during inference, while DeepSeek-R1 \citep{Guo_2025} achieves similar effects through reinforcement learning. \citet{snell2024scaling} demonstrate that scaling inference-time compute can outperform parameter scaling on reasoning benchmarks. This success has sparked a natural but largely untested assumption: enhanced reasoning capabilities will universally translate to superior performance in complex, open-ended domains, such as creative writing. However, whether these gains transfer to subjective generative tasks remains an open question. For instance, DeepSeek-R1 serves as a direct reasoning RL upgrade built upon DeepSeek-V3 \cite{liu2024deepseek}, allowing for the isolation of the reasoning RL phase's impact on narrative quality. Anecdotal concerns and widespread public sentiment suggest a preference for GPT-4o's \cite{hurst2024gpt} conversational style over GPT-5's outputs, raising the possibility that reasoning mechanisms introduce negative stylistic artifacts that harm human interaction and narrative resonance. 

% Systematic evaluation on narrative and psychological dimensions is lacking, particularly as frontier models may have entered an "evaluation plateau" where objective flaws are rare and individual human subjectivity dictates preference.


% \subsection{LLM-as-a-Judge: From Uniform Alignment to Personalized Evaluation}

% While the “LLM-as-a-judge” paradigm \citep{zheng2023judgingllmasajudgemtbenchchatbot} provides a scalable alternative to human annotation, existing frameworks often exhibit systematic misalignment due to inherent biases—such as position, verbosity, and self-enhancement—as well as their reliance on uniform, one-size-fits-all scoring rubrics \citep{li-etal-2025-generation}. A central driver of this misalignment is the fundamentally subjective nature of evaluation \cite{dong-etal-2024-llm}, which depends on user-specific personas \cite{dong-etal-2024-llm} and multi-session contextual preferences \cite{liu-etal-2025-persona}. Consequently, model-centric evaluation heuristics often fail to capture the nuanced, preference-driven dynamics underlying human judgment.

% Traditionally, many evaluators adopt Likert scales to assign absolute, pointwise ratings. However, such scales often struggle to capture fine-grained distinctions and are susceptible to calibration inconsistencies across judges. To address these limitations, \citet{liu2024aligning} propose pairwise evaluation, which replaces absolute scoring with uncertainty-aware comparative ranking and better aligns with human judgment. Nevertheless, recent findings indicate that the comparative nature of pairwise evaluation can itself amplify certain biases \cite{jeong-etal-2025-comparative}.

% Motivated by these limitations, we further identify a bias toward reasoning-model outputs, highlighting the need for personalized evaluation and bridging the gap between rigid, model-centric metrics and nuanced, preference-driven human judgment.


% \subsection{Subjective Disagreement and Annotator Heterogeneity}
% Research on disagreement and annotator heterogeneity in LLM evaluation has shifted from treating labeling variance as noise to recognizing it as a meaningful signal of subjective human values and task ambiguity \citep{kirk2024prism, sandri-etal-2023-dont}. Prior work shows that standard alignment methods, such as DPO \cite{rafailov2023direct}, often fail to capture diversity across user groups, resulting in “majority-rule” biases that marginalize minority perspectives. To address this limitation, recent approaches—including pluralistic alignment frameworks \cite{chen2024pal}, distributional reward models \cite{dorka2024quantile}, and subjectivity-aware evaluation metrics \cite{fleisig-etal-2023-majority}—explicitly model systematic differences in how individuals and demographics evaluate content. By incorporating annotator-specific context, these methods move toward representing the inherent diversity of human judgment rather than enforcing a single consensus. In subjective NLP tasks, low inter-annotator agreement should not be interpreted as annotation failure; instead, it often reflects genuine differences in evaluative criteria \citep{clark-etal-2021-thats, sandri-etal-2023-dont}. Building on this perspective, our analysis suggests that variation in how annotators weight PDS dimensions may contribute to the observed disagreement.

==> content_v2/03_Dataset.tex <==
\section{\textsc{PsychDepth Reasoning} dataset}
\label{sec:dataset}

% In order to measure the effects of reasoning post-training on creative writing, we construct a \textsc{PsychDepth Reasoning} dataset  comprised of 120 stories organized into pairs to facilitate comparisons generated from 20 carefully curated premises.

To examine how reasoning-oriented post-training affects creative writing, we constructed \textsc{PsychDepth Reasoning}. This dataset contains 120 stories organized into 60 prompt-matched pairs from 20 carefully curated premises.

\paragraph{Defining ``reasoning-enhanced.''}
In this paper, we use \textit{reasoning-enhanced} to refer to models whose post-training emphasizes deliberative reasoning behavior, typically via reinforcement learning or related reasoning-oriented optimization. In our study, this includes DeepSeek-R1, which uses reasoning-oriented RL \citep{Guo_2025}, and GPT-5, which uses extended chain-of-thought inference \citep{singh2025openaigpt5card}. We use \textit{base} model to refer to counterparts without such reasoning-oriented post-training, i.e. DeepSeek-V3 and GPT-4o.

\paragraph{Premise selection.}
To elicit psychological depth, we curated 20 premises that provide contextual framing for character development while leaving the narrative direction open. We sourced 15 premises from Reddit’s r/WritingPrompts\footnote{\url{https://www.reddit.com/r/WritingPrompts}}, a highly popular online community known for its thematic diversity and structured, high-concept story prompts, and 5 premises from Reedsy\footnote{\url{https://reedsy.com/creative-writing-prompts/}}, a professional platform offering traditional literary prompts. To prevent data contamination, we restricted Reddit selection to prompts posted after the known training-data cutoff dates for GPT-5 and DeepSeek-R1, then ranked candidates by all-time upvotes and manually filtered for quality. The full list of all 20 premises appears in Appendix~\ref{app:premises}.

\paragraph{Model pairings and pair construction.}
We selected the GPT and DeepSeek model families to compare prompt-matched story outputs from reasoning and non-reasoning models. For each premise, we paired one reasoning-model story with one base-model story from the same family. All stories were generated with a common zero-shot story-writing template, with only limited family-specific wording adjustments for word-count compliance. Full prompts and sampling settings appear in Appendix~\ref{app:generation}.


% \begin{description}
%     \item[DeepSeek-R1 vs.\ DeepSeek-V3 (20 pairs).] \hfill \\
%     % DeepSeek-R1 is a direct reasoning RL upgrade built upon DeepSeek-V3, providing a tightly controlled comparison that isolates the impact of the reasoning RL phase on narrative quality.
%     DeepSeek-R1, an RL upgrade of DeepSeek-V3, provides a controlled comparison isolating the impact of reasoning RL on narrative quality.

%     \item[GPT-5 vs.\ GPT-4o (40 pairs).] \hfill \\
%     GPT-5 is one of the most widely used frontier reasoning models. We evaluate it against GPT-4o under two distinct reasoning budget settings, defined as the number of reasoning tokens generated prior to the final response. These include \textbf{GPT-5 (auto)}, where the model autonomously determines the reasoning length via its built-in implementation, and \textbf{GPT-5 (high)} (n=20 pairs each), to test whether increased reasoning compute affects perceived psychological depth.

% \end{description}

\textbf{DeepSeek-R1}, an RL upgrade of \textbf{DeepSeek-V3}, provides a controlled comparison isolating the impact of reasoning RL on narrative quality (20 pairs). For the GPT family, we evaluated \textbf{GPT-5}, one of the most widely used frontier reasoning models, against \textbf{GPT-4o} under two distinct reasoning budget settings, defined as the number of reasoning tokens generated prior to the final response: \textbf{GPT-5 (auto)}, where the model autonomously determines the reasoning length ($7{,}846 \pm 3{,}117$ reasoning tokens on average), and \textbf{GPT-5 (high)} ($11{,}606 \pm 3{,}557$ reasoning tokens, roughly $1.5 \times$ the auto budget), with 20 pairs each, to test whether increased reasoning compute affects perceived psychological depth.


==> content_v2/04_Human_Study.tex <==
\section{Human study}
\label{sec:human}
We adapted the \citet{harelcanada2024measuringpsychologicaldepthlanguage} framework to a blinded pairwise protocol. The Institutional Review Board (IRB) deemed this study exempt.

\subsection{Annotator recruitment and training}
\label{sec:training}

We recruited undergraduate students from the English and Psychology departments at a large research university using targeted interest forms. From 70 applicants, we selected the 7 most promising candidates based on English proficiency, interest in the research, and experience reviewing short stories, with cohort size determined by budget constraints. 
% Our goal was to engage semi-expert annotators with relevant literary and psychological backgrounds, bridging the gap between crowdsourced workers and professional experts.

We conducted comprehensive online onboarding sessions covering the five PDS metrics and our custom Label Studio annotation interface \citep{LabelStudio}. The participants then independently completed the annotations in seven days and received \$100 each.

\subsection{Annotation protocol}
\label{sec:protocol}

For each of the 60 pairs, two stories were presented side-by-side in a randomized order, with the PDS rubric definitions shown at the top of the page. For each pair, annotators provided six pairwise preference judgments: one for each of the five PDS dimensions (authenticity, empathy, engagement, emotion provocation, and narrative complexity) and one overall preference judgment (see Appendix~\ref{app:interface}). Annotators could also submit free-text justifications. This produced $7 \times 60 \times 6 = 2{,}520$ pairwise preference judgments, along with 112 free-text justifications. To monitor annotation quality, we logged per-pair completion times and conducted a Leave-One-Annotator-Out (LOAO) stability analysis and administered a post-study survey; all quality checks are reported in Appendix~\ref{app:annotator_time} and~\ref{app:post_survey}.

% \subsection{Annotation Quality Checks}

% We logged annotation times per pair for each annotator and present the full plots in Appendix~
% \ref{app:annotator_time}. The median annotation time ranged from 108 to 418 seconds across annotators (Figure~\ref{fig:annotation_time_dist}). Annotator~6 was a notable speed outlier (median 108s), consistent with their background as an English major and professional reader. Their pacing remained highly consistent over time (Figure~\ref{fig:annotation_time_trend}).

% To verify that no single annotator drove the aggregate results, we conducted a Leave-One-Annotator-Out (LOAO) stability analysis (Figure~\ref{fig:loao_stability}). Removing any single annotator, including Annotator~6, caused only a $2$--$4\%$ shift in overall win rates, confirming that each annotator contributed a valid, stable signal.



==> content_v2/05_LLM_Judge.tex <==
\section{LLM-as-a-Judge evaluator}
\label{sec:auto}

To compare automatic and human judgments, we constructed an LLM-as-a-Judge pipeline that extends a zero-shot evaluation framework to a controlled few-shot paradigm.

\subsection{Evaluator construction}

% Our pipeline uses DSPy \citep{dspy} to enforce structured output control, ensuring that LLM judges consistently return 1-to-5 Likert scale ratings. We retain the Mixture-of-Personas (MoP) prompting strategy from the foundational PDS study \citep{harelcanada2024measuringpsychologicaldepthlanguage}, which primes evaluators with distinct analytical perspectives (e.g., literary critic, psychologist) to improve assessment of multifaceted subjective criteria \citep{salewski2023context}.

Our pipeline uses DSPy \citep{dspy} to enforce structured output control and thereby ensures that LLM judges return 1-to-5 Likert ratings. We retained the Mixture-of-Personas prompting strategy from the original PDS study. This strategy primes evaluators with distinct analytical perspectives and draws on prior work showing that in-context impersonation can shape LLM performance and reveal different strengths and biases \citep{salewski2023context}. To construct in-context demonstrations, we used the original 97-story dataset and its human annotations from \citet{harelcanada2024measuringpsychologicaldepthlanguage}. We partitioned the dataset into a 20\% demonstration pool and an 80\% validation split. We then selected representative few-shot examples from the demonstration pool by applying $k$-means clustering to the PDS score vectors, drawing on prior selective-annotation work that emphasizes diverse, representative examples for in-context learning \citep{su2022selective}.

We used a scalar-rating evaluator rather than a directly pairwise-trained judge because the original PDS dataset provides scalar supervision with strong inter-annotator agreement. With this formulation, we can both construct calibrated few-shot prompts and validate the evaluator quantitatively against held-out human ratings before deployment.

\subsection{Evaluator selection and validation}
\label{sec:validation}

% We validate evaluator performance on the 80\% held-out split, measuring Spearman correlation ($\rho$) with average human ratings. We experiment across multiple base models---Llama~3.1~70B, Llama~3.3~70B \citep{grattafiori2024llama3herdmodels}, and Qwen3.5-397B \citep{qwen35blog}---varying demonstration counts ($k \in \{5, 7, 10\}$) and testing Chain-of-Thought (CoT) prompting \citep{wei2022chain}. Table~\ref{tab:evaluator_comparison_transposed} reports the full breakdown. The best configuration is Llama~3.1~70B with 7 demonstrations, achieving the highest overall average correlation ($\rho = 0.606$). However, no single configuration dominates across all dimensions, motivating the ensemble approach described below.

We validated evaluator performance on the 80\% held-out split by measuring Spearman correlation ($\rho$) with average human ratings. We tested multiple base models---Llama~3.1~70B, Llama~3.3~70B \citep{grattafiori2024llama3herdmodels}, and Qwen3.5-397B \citep{qwen35blog}---across different demonstration counts ($k \in \{5, 7, 10\}$) and with or without Chain-of-Thought prompting \citep{wei2022chain}. Table~\ref{tab:evaluator_comparison_transposed} reports the full breakdown. Llama~3.1~70B with 7 demonstrations achieved the highest overall average correlation ($\rho = 0.606$). However, no single configuration performs best across all dimensions: CoT performs best on narrative complexity ($\rho = 0.664$), Qwen3.5 on engagement ($\rho = 0.564$), and Llama~3.3~70B on empathy ($\rho = 0.702$).

\begin{table}[t]
\caption{Evaluator Spearman correlation ($\rho$) with human annotations across PDS dimensions. Bold values indicate the best configuration in each upper-section column. The best dimension-specific configurations form the ensemble (bottom row).}
\label{tab:evaluator_comparison_transposed}
\centering
\small
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcccccc}
\toprule
\textbf{Evaluator} & \textbf{AUT} & \textbf{PROV} & \textbf{EMP} & \textbf{ENG} & \textbf{NCOM} & \textbf{Overall} \\
\midrule
Llama 3.1 70B demo=7   & 0.576 & 0.674 & 0.637 & 0.507 & 0.637 & \textbf{0.606} \\
Llama 3.1 70B demo=5   & \textbf{0.588} & 0.655 & 0.596 & 0.450 & 0.575 & 0.573 \\
Llama 3.1 70B demo=10  & 0.561 & \textbf{0.702} & 0.671 & 0.387 & 0.568 & 0.578 \\
Llama 3.3 70B demo=10  & 0.580 & 0.676 & \textbf{0.702} & 0.407 & 0.550 & 0.583 \\
Qwen 3.5 397B demo=7      & 0.511 & 0.663 & 0.602 & \textbf{0.564} & 0.496 & 0.567 \\
Llama 3.1 70B CoT demo=10 & 0.499 & 0.627 & 0.658 & 0.356 & \textbf{0.664} & 0.561 \\
\midrule
\textbf{Ensemble} & 0.588 & 0.702 & 0.702 & 0.564 & 0.664 & 0.646 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Ensemble evaluator}

To maximize reliability, we constructed a heterogeneous ensemble that assigns each PDS metric to its best-performing model configuration on the validation split (Table~\ref{tab:evaluator_comparison_transposed}, bottom row). The ensemble achieves $\rho = 0.646$, outperforming every single-model configuration as well as the zero-shot approach of \citet{harelcanada2024measuringpsychologicaldepthlanguage} ($\rho \approx 0.51$ with GPT-4o). At inference time, we converted scalar Likert outputs into pairwise comparisons: for each of the 60 pairs, the ensemble evaluated both stories independently and selected the higher-scoring story as the preference. When both stories receive the same score on a dimension, we broke ties randomly. In practice, ties were rare: the overall preference metric has no ties across the 60 pairs, and most other dimensions have 0--3 ties. Authenticity is the main exception, with 16 ties out of 60. Full tie statistics appear in Appendix~\ref{sec:appendix-ties}.

% \paragraph{Scope and Limitations.}
% The evaluator was validated on scalar ratings from an older dataset and applied here to pairwise frontier comparisons, introducing a potential distributional mismatch. We use the evaluator as \emph{supporting analysis} to contrast with human judgments, not as a replacement for human evaluation.


==> content_v2/06_Results_Analysis.tex <==
\section{Results and analysis}
\label{sec:results}

% We organize our analysis around the three research questions (\textbf{RQ1}, \textbf{RQ2}, \textbf{RQ3}) from Section~\ref{sec:intro}. We first examine human preferences across model families and PDS dimensions (\S\ref{sec:rq1}), then turn to annotator disagreement (\S\ref{sec:rq2}), and finally compare human judgments with the automatic evaluator (\S\ref{sec:rq3}). We close with a brief discussion of implications for evaluating frontier creative generation (\S\ref{sec:implications}).

We organized our analysis around the three research questions from Section~\ref{sec:intro}. Section~\ref{sec:rq1} addresses \textbf{RQ1} (human preferences across model families and PDS dimensions), Section~\ref{sec:rq2} addresses \textbf{RQ2} (sources of annotator disagreement), and Section~\ref{sec:rq3} addresses \textbf{RQ3} (comparison with the LLM-as-Judge evaluator). We close with a brief discussion of implications for evaluating frontier creative generation in Section~\ref{sec:implications}.

\subsection{Human preferences do not show a universal reasoning advantage}
\label{sec:rq1}
% Answers RQ1

% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Pair} & \textbf{Pref.} & \textbf{All 6} \\
% \midrule
% GPT-5 (auto) vs.\ 4o & 60.0\% & 61.4\% \\
% GPT-5 (high) vs.\ 4o & 62.9\% & 60.8\% \\
% DeepSeek-R1 vs.\ V3 & 42.9\% & 50.5\% \\
% \midrule
% \textbf{Overall} & \textbf{55.2\%} & \textbf{57.6\%} \\
% \bottomrule
% \end{tabular}
% \caption{Human preference rate for the reasoning model. \textbf{Pref.}\ = overall preference metric only; \textbf{All~6} = pooled across all six evaluation dimensions. Rates represent the proportion of annotator votes favoring the reasoning model ($n = 7$ annotators $\times$ 20 pairs per matchup).}
% \label{tab:human_pref}
% \end{table}

\begin{table}[t]
\caption{Preference rates for reasoning models: human annotators vs.\ LLM-as-Judge evaluator. Pref.\ = overall preference. $\Delta$ = mean Likert score difference (reasoning $-$ non-reasoning); $d$ = Cohen's $d$.}
\label{tab:pref_comparison}
\centering
\small
\begin{tabular}{l cc ccc}
\toprule
& \textbf{Human} & \textbf{LLM Judge} & \multicolumn{3}{c}{\textbf{LLM Judge Bias}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-6}
\textbf{Pair} & \textbf{Pref.} & \textbf{Pref.} & \textbf{$\Delta$} & \textbf{$d$} & \textbf{$p$} \\
\midrule
GPT-5 (auto) vs.\ 4o & 60.0\% & 100.0\% & $+0.518$ & 1.14 & $<\!.001$ \\
GPT-5 (high) vs.\ 4o & 62.9\% & 100.0\% & $+0.500$ & 1.12 & $<\!.001$ \\
DeepSeek-R1 vs.\ V3 & 42.9\% & 95.0\% & $+0.214$ & 0.68 & $<\!.001$ \\
\midrule
\textbf{Overall} & 55.2\% & 98.3\% & $+0.411$ & 0.95 & $<\!.001$ \\
\bottomrule
\end{tabular}
\end{table}

Human preferences diverge across model families. Although reasoning models receive 55.2\% of preference votes overall, this aggregate obscures a sharp family-level split (Table~\ref{tab:pref_comparison}). Within the GPT family, annotators modestly prefer GPT-5 over GPT-4o (60.0\% for “auto”, 62.9\% for “high” reasoning effort setting). In contrast, DeepSeek-R1 trails DeepSeek-V3, receiving only 42.9\% of preference votes. 

% TODO: Forest plot with per-metric, per-family confidence intervals to show
% which metric × family combinations drive the effect and which are consistent
% with chance. This would strengthen the claim that the effect is not uniform.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.6\textwidth]{figs/fig1_forest_plot.png}
%     \caption{Human preference rates for the reasoning model by model family and PDS dimension, with 95\% Wilson confidence intervals. The dashed line indicates 50\% (no preference). GPT-5 pairings show more consistently pro-reasoning preferences, especially on affective dimensions, whereas DeepSeek-R1 vs V3 is mixed and often overlaps with the no-preference line.}
%     \label{fig:forest_plot}
% \end{figure}

\begin{table}
\caption{Human preference for reasoning models by model family and PDS dimension. Entries show preference rate with 95\% Wilson CI ($n=140$ per cell). Rates above 50\% favor the reasoning model; $\uparrow$ and $\downarrow$ indicate intervals entirely above or below 50\%, respectively.}
\label{tab:human_by_dimension}
\centering
\small
\begin{tabular}{l ccc}
\toprule
& \textbf{DeepSeek-R1} & \textbf{GPT-5 (auto)} & \textbf{GPT-5 (high)} \\
\textbf{Dimension} & \textbf{vs.\ V3} & \textbf{vs.\ 4o} & \textbf{vs.\ 4o} \\
\midrule
Authenticity & \shortstack{47.9\%\\{[39.8, 56.1]}} & \shortstack{55.7\%\\{[47.4, 63.7]}} & \shortstack{52.1\%\\{[43.9, 60.2]}} \\
Empathy & \shortstack{53.2\%\\{[45.0, 61.3]}} & \shortstack{68.6\% $\uparrow$\\{[60.5, 75.7]}} & \shortstack{69.3\% $\uparrow$\\{[61.2, 76.3]}} \\
Engagement & \shortstack{39.3\% $\downarrow$\\{[31.6, 47.6]}} & \shortstack{58.6\% $\uparrow$\\{[50.3, 66.4]}} & \shortstack{65.0\% $\uparrow$\\{[56.8, 72.4]}} \\
Emotion Prov. & \shortstack{61.4\% $\uparrow$\\{[53.2, 69.1]}} & \shortstack{70.7\% $\uparrow$\\{[62.7, 77.6]}} & \shortstack{62.9\% $\uparrow$\\{[54.6, 70.4]}} \\
Narr.\ Complexity & \shortstack{58.6\% $\uparrow$\\{[50.3, 66.4]}} & \shortstack{55.0\%\\{[46.7, 63.0]}} & \shortstack{52.9\%\\{[44.6, 60.9]}} \\
\midrule
\textbf{Overall Preference} & \shortstack{42.9\%\\{[35.0, 51.1]}} & \shortstack{60.0\% $\uparrow$\\{[51.7, 67.7]}} & \shortstack{62.9\% $\uparrow$\\{[54.6, 70.4]}} \\
% \midrule
% \textbf{All (pooled)} & 50.5\% \scriptsize{[47.2, 53.9]} & 61.4\% \scriptsize{[58.1, 64.7]} & 60.8\% \scriptsize{[57.5, 64.1]} \\
\bottomrule
\end{tabular}
\end{table}

The same divergence appears across PDS dimensions. Table~\ref{tab:human_by_dimension} shows that the GPT-5 pairings were consistently above 50\% on affective dimensions, especially \textit{emotion provocation} and \textit{empathy}, whereas DeepSeek-R1 vs.\ V3 exhibited mixed effects across dimensions and was notably disfavored on \textit{engagement} (39.3\%). The aggregate 55.2\% therefore should not be read as a universal reasoning advantage. Figure~\ref{fig:annotator_heatmap} visualizes this variation across individual annotators, model families, and PDS dimensions. Individual annotators range from strong pro-reasoning (Annotator 7, 80\%) to strong pro-base (Annotator 1, 36.7\%), underscoring that the aggregate masks substantial reader-level disagreement.

\begin{figure}
\centering
\includegraphics[width=0.9\textwidth]{figs/reasoning_preference_all_ensemble.png}
\caption{Preference rates for reasoning models across 7 individual human annotators, the human average, and the ensemble LLM judge.}
\label{fig:annotator_heatmap}
\end{figure}

\paragraph{Takeaway.} Reasoning does not have a universal effect on psychological depth. The direction and magnitude of human preference depend on both model family and the PDS dimension under evaluation.


\subsection{Inter-annotator disagreement reflects evaluative subjectivity}
\label{sec:rq2}
% Answers RQ2

\begin{table}[h]
\caption{Inter-annotator agreement across 60 pairs and 7 annotators. Raw = average pairwise agreement rate. Bold indicates the highest value among dimensions in each column.}
\label{tab:iaa}
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Metric} & \textbf{Fleiss' $\kappa$} & \textbf{Kripp.\ $\alpha$} & \textbf{Raw} \\
\midrule
Authenticity & 0.035 & 0.037 & 52.5\% \\
Emotion Prov. & 0.080 & 0.082 & 54.1\% \\
Empathy & \textbf{0.182} & \textbf{0.185} & \textbf{59.1\%} \\
Engagement & 0.059 & 0.061 & 53.3\% \\
Narr.\ Complexity & 0.016 & 0.018 & 52.1\% \\
Preference & 0.035 & 0.038 & 51.9\% \\
\midrule
\textbf{Average} & 0.068 & 0.070 & 53.8\% \\
\bottomrule
\end{tabular}
\end{table}

% \begin{table*}[t]
% \centering
% \footnotesize
% \renewcommand{\arraystretch}{1.2}
% \begin{tabularx}{\textwidth}{p{2.5cm} c X c c X}
% \toprule
% \textbf{Premise (Pair)} & \multicolumn{2}{c}{\textbf{Annotator 1}} & \textbf{Agr.} & \multicolumn{2}{c}{\textbf{Annotator 7}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){5-6}
% & \textbf{Pref.} & \textbf{Comment} & & \textbf{Pref.} & \textbf{Comment} \\
% \midrule

% ``Hide something from your reader\ldots'' (36)
% & A
% & ``B: Second person, generally confusing but ominous.''
% & 4/6
% & B
% & ``Story~A doesn't `hide' very much at all\ldots{} Story~B sets up a larger secret. Flow mimics human experience and invokes more empathy towards loss.''
% \\
% \addlinespace

% ``Humans viewed like Witches/Warlocks\ldots'' (27)
% & A
% & ``A: like a prologue. \newline B: prose, very nonsensical.''
% & 1/6
% & B
% & ``B is very cute and I enjoy seeing the concept in action. Story~A feels like the setup to the story that should be present.''
% \\
% \addlinespace

% ``The king has a large problem\ldots'' (24)
% & A
% & ``A: good imagery, dialogue. \newline B: interesting parallels, odd tone.''
% & 2/6
% & B
% & ``A is a step by step of the prompt given. B builds up characters, establishes risk, and is authentic\ldots{} genuinely something I myself would write.''
% \\

% \bottomrule
% \end{tabularx}
% \caption{Annotator~1 vs.\ Annotator~7 on three story pairs where they disagree on overall preference. \textbf{Agr.} denotes the number of six evaluation dimensions (five PDS dimensions plus overall preference) on which the two annotators agreed.}
% \label{tab:ann1_ann7}
% \end{table*}

Inter-annotator agreement is extremely low (Table~\ref{tab:iaa}): Krippendorff's $\alpha = 0.070$ on average, with raw pairwise agreement barely above the $50\%$ expected by chance. This is a dramatic drop from the $\alpha \approx 0.72$ reported by \citet{harelcanada2024measuringpsychologicaldepthlanguage} using the same PDS rubric. However, the two evaluation settings differ substantially: the original PDS study validated its rubric on a dataset spanning Reddit-collected human stories and LLM generations from 2023-era models, including many weaker open-source systems, where quality gaps were large enough to support clear discrimination. Our setting is considerably more challenging: both stories in each pair are generated by frontier models, and our comparisons isolate only the effect of reasoning-oriented post-training, producing much smaller quality differences. That the observed improvements are subtle rather than obvious means that preferences are more likely to reflect individual reader subjectivity than a detectable quality gap. This low agreement is not driven by a single model matchup; Appendix~\ref{app:iaa_breakdown} (Table~\ref{tab:iaa_breakdown}) shows similarly weak, and sometimes near-zero or negative, agreement across all three pairings.

% While inter-annotator agreement is low, this disparity does not imply that annotators were careless or incompetent. Several lines of evidence argue against annotation failure:

% \begin{itemize}
%     \item \textbf{Timing consistency.} Annotators spent substantial time per pair (median 108--418s), with stable pacing over the session (Figures~\ref{fig:annotation_time_dist}--\ref{fig:annotation_time_trend}).
%     \item \textbf{LOAO stability.} Removing any single annotator shifts the aggregate win rate by only $2$--$4\%$ (Figure~\ref{fig:loao_stability}), confirming that no individual drives the results.
%     % TODO: Add comment coverage statistics.
% \end{itemize}

As described in Section~\ref{sec:training}, we took careful steps to ensure high annotation quality. Multiple quality checks, including timing consistency and LOAO stability (Appendix~\ref{app:annotator_time}), confirm that the annotators engaged substantively with the task, spending a median of 108–418 seconds per pair with stable pace throughout. Removing any single annotator changes the aggregate win rate by only $2$--$4\%$ (Figure~\ref{fig:loao_stability}), confirming no individual drives the results.

Given that the disagreement does not appear to stem from annotation failure, we investigated possible sources of this divergence. The annotator-level heatmap in Figure~\ref{fig:annotator_heatmap} reveals a suggestive pattern: Annotator~7 strongly favors reasoning models ($70$--$80\%$ across most dimensions), while Annotator~1 prefers the non-reasoning counterparts ($27.5\%$ for engagement, $32.5\%$ for overall preference). This pattern motivates a deeper look into the decision logic of individual annotators. Specifically, we employ regression analysis to identify which dimensions most strongly predict the overall preference, and calculate intra-annotator Cohen’s $\kappa$ to quantify the alignment between dimensional ratings and the overall preference.
\newline
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/regression_and_cohen.png}
    \caption{Hierarchical clustering of annotator archetypes and PDS dimensions. \textbf{Left:} Logistic-regression coefficient profiles, where weights quantify each dimension's influence on overall preference. \textbf{Right:} Intra-annotator Cohen’s $\kappa$ between dimensional and overall judgments.
    }
    \label{fig:annotator_clustering}
\end{figure}

\paragraph{Logistic regression weight analysis.}

We fit individual logistic regression models, \[
P(y_{a,i}=1 \mid x_{a,i}) = \sigma\!\left(\beta_{a,0} + \sum_{m \in \mathcal{M}} \beta_{a,m} x_{a,i,m}\right),
\] where \(\beta_{a,m}\) captures how dimension $m$ predicts an annotator's overall preference.

Hierarchical clustering of the coefficients (Figure~\ref{fig:annotator_clustering}, left) reveals substantial heterogeneity in dimensional aggregation. Weighting priorities vary from affective dimensions to structural ones. In particular, Annotators~1 and~3 form a cluster characterized by relatively stronger reliance on engagement and authenticity, whereas Annotators~4 and~7 assign broadly high positive weights across multiple dimensions, showing a more balanced aggregation strategy.


\paragraph{Cohen's $\kappa$ analysis.} In parallel with the logistic regression profiles, we calculate Cohen’s $\kappa$ between each single-dimension preference and the overall preference (Figure~\ref{fig:annotator_clustering}, right). The two clustering structures are highly similar and share the same innermost sub-clusters: key annotator sub-clusters are ((Ann~1, Ann~3), Ann~2) and (Ann~4, Ann~7), while empathy and emotion provocation are the most closely clustered dimensions. Generally, higher Cohen's $\kappa$ agreement corresponds to stronger predictive influence (larger \(\beta_{a,m}\)) in the regression models. This confirms that low inter-annotator agreement is driven by divergent weighting schemes rather than random judgment errors. 


% TODO: Annotator clustering / archetypes analysis.

% TODO: Ann 1 vs Ann 7 qualitative example from free-text comments,
% illustrating concretely how two annotators evaluate the same story pair
% from different but valid perspectives.

Qualitative comparison of annotator comments further supports this interpretation. Annotators frequently disagree not because they overlook the same features, but because they prioritize different qualities, for instance valuing narrative clarity over emotional immediacy, or vice versa. These trade-offs reflect coherent evaluative strategies rather than random disagreement. Detailed comment examples are provided in Appendix~\ref{app:annotator_comment}.

\paragraph{Takeaway.} Annotators diverge in how they weight psychological-depth dimensions when forming overall preferences. The narrow quality gap between frontier model pairs, substantially smaller than in the original PDS validation setting, means that preferences are more likely to reflect genuine evaluative subjectivity than detectable quality differences. % Multiple quality checks， including timing consistency, comment coverage, and LOAO stability, confirm that this disagreement is not attributable to annotation failure. Exploratory analysis suggests that one source of this subjectivity may be that annotators differ in how they weight psychological-depth dimensions when forming overall preferences.

\subsection{LLM judges flatten human heterogeneity}
\label{sec:rq3}
% Answers RQ3

The LLM judge presents a drastically different picture (Table~\ref{tab:pref_comparison}, LLM Judge columns). It preferred the reasoning model 98.3\% of the time, nearly doubling the human preference rate of 55.2\%. For DeepSeek, where humans actually preferred V3, the evaluator still favored R1 at 95.0\%. This bias is not an artifact of the ensemble construction: all five individual judge configurations preferred the reasoning model on average (Appendix~\ref{sec:appendix-judge-breakdown}).

Figure~\ref{fig:annotator_heatmap} juxtaposes the per-annotator human preferences with the LLM-as-Judge evaluator's scores. The human columns display a heterogeneous patchwork of preferences, while the "LLM Judge" column is nearly uniformly saturated in favor of reasoning models. Per-model-family breakdowns (Appendix~\ref{sec:appendix-heatmaps}) and a detailed case study of one pair where human and LLM preferences sharply diverge (Appendix~\ref{sec:appendix-case}) further illustrate this contrast. The evaluator did not recover the family-level or annotator-level variation present in the human data but flattened it. This misalignment is further quantified in Appendix~\ref{app:agreement} (Figure~\ref{fig:auto_agreement}): overall human–judge agreement averages only 64.2\%, dropping to chance level for DeepSeek and just 30.0\% on DeepSeek preference alone. This bias is quantified by score differences in Table~\ref{tab:pref_comparison}: the evaluator assigns reasoning models a mean score advantage of $+0.411$, most pronounced for GPT-5 ($d \approx 1.1$) and attenuated but still significant for DeepSeek ($d = 0.68$).


\paragraph{Takeaway.} Although the LLM-as-Judge evaluator achieved strong agreement with human annotations in the original PDS setting, it exhibits a pronounced pro-reasoning bias on frontier story pairs, compressing family- and annotator-level variation into a near-uniform preference for reasoning models that diverges from the heterogeneous human signal.

\subsection{Implications for evaluating frontier creative generation}
\label{sec:implications}

% Our results carry several practical implications:

\paragraph{Annotator heterogeneity should be modeled.} When agreement is near chance, the ``majority vote'' is not a stable consensus but a fragile artifact of the specific annotator sample. Future work should characterize the \emph{distribution} of human preferences, including annotator archetypes and their metric-weighting profiles, rather than collapsing into a single win-rate.

\paragraph{LLM judges require human-grounded interpretation.} Prior work has documented systematic failure modes in LLM judges, including position, verbosity, and self-enhancement biases \citep{li-etal-2025-generation, 10.5555/3737916.3740113, stureborg2024large, wang2024large}. Our findings reveal an additional mode: a strong pro-reasoning bias, with the ensemble evaluator preferring reasoning models 98.3\% of the time compared to the humans' 55.2\%. This is all the more notable because most of our evaluator models (Llama 3.1, Llama 3.3) predate the reasoning era of LLMs and do not plausibly favor reasoning-model outputs due to training data exposure to synthetic reasoning traces. One plausible explanation is that the evaluator is more sensitive than humans to stylistic artifacts associated with reasoning-oriented generation, although the exact source of this skew is left to future work.

==> content_v2/07_Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% We present a controlled study of whether reasoning-enhanced LLMs produce stories with greater psychological depth, evaluating 60 story pairs across three frontier model matchups with seven human annotators and an ensemble LLM-as-a-Judge.

% Our findings show that reasoning enhancement can improve human-perceived psychological depth in some comparisons, particularly within the GPT-5 vs.\ GPT-4o family, but these gains are not uniform across model families or readers. DeepSeek-R1 falls behind V3, demonstrating that reasoning-oriented post-training does not universally benefit creative generation. Human disagreement, rather than reflecting annotation failure, appears to stem from genuine evaluative subjectivity; exploratory analysis suggests that differences in how readers weight psychological-depth dimensions may be one contributing factor. The automatic evaluator compresses this heterogeneity into a stronger and more homogeneous pro-reasoning signal ($98.3\%$ vs.\ humans' $55.2\%$), underscoring the risk of relying on LLM judges as proxies for human literary preference.
We evaluated whether reasoning-enhanced LLMs produce stories with greater psychological depth across 60 frontier story pairs, seven human annotators, and an ensemble LLM-as-a-Judge. Reasoning enhancement improved perceived depth in some comparisons (GPT-5 vs. GPT-4o) but not others (DeepSeek-R1 vs. V3), demonstrating that reasoning-oriented post-training does not universally benefit creative generation. Human disagreement reflected genuine evaluative subjectivity, with annotators applying distinct weighting schemes across PDS dimensions rather than responding to a shared quality difference. The LLM-as-Judge evaluator compressed this heterogeneity into a near-uniform pro-reasoning signal (98.3\% vs. humans' 55.2\%), underscoring the risk of relying on LLM judges for creative evaluation.

% \paragraph{Future Work.}
% Several directions could strengthen and extend these findings:
% \begin{itemize}
%     \item \textbf{Intra-rater reliability}: Repeated-rating studies to separate genuine preference instability from inter-rater disagreement.
%     \item \textbf{Pairwise-trained judges}: Evaluators trained directly on pairwise preference data rather than adapted from scalar ratings.
%     \item \textbf{Larger annotator pools}: More diverse cohorts to better characterize the distribution of evaluative priorities.
%     \item \textbf{Annotator profile modeling}: Explicit modeling of annotator archetypes and their metric-weighting schemes, moving beyond aggregate win-rates toward distributional evaluation frameworks.
% \end{itemize}

\section*{Limitations}

\paragraph{Scale.}
With 20 premises and 60 pairwise comparisons, our evaluation can identify large-effect biases but lacks the statistical power to detect smaller human preference effects.

\paragraph{Model coverage.} Our findings are specific to the tested models (GPT-5, GPT-4o, DeepSeek-R1, DeepSeek-V3) and may not generalize to other reasoning-enhanced architectures.

\paragraph{Annotator demographics.} All annotators are undergraduates from English and Psychology departments at a single university ($n = 7$), which may introduce demographic and cultural biases.

\paragraph{Task specificity.} We evaluate only short-story generation. Whether the observed patterns hold for other creative tasks (poetry, dialogue, long-form fiction) remains open.

\paragraph{Evaluator generalization.} The ensemble evaluator was validated on scalar ratings from a 97-story dataset predating the frontier models tested here and applied to pairwise frontier comparisons, introducing a potential distributional mismatch. We therefore use the evaluator as \emph{supporting analysis} to contrast with, rather than replace, human judgments.

\section*{Ethics statement}

This study was reviewed and determined to be exempt by our Institutional Review Board. All human annotators were compensated for their time and provided informed consent. The generated stories are fictional and contain no personally identifiable information. We acknowledge that our findings regarding LLM judge bias have implications for the responsible deployment of LLM-as-Judge evaluation systems.


==> content_workshop/00_abstract.tex <==
\begin{abstract}
LLM judges are increasingly used to evaluate open-ended generation, yet development-set correlation may not guarantee valid measurement when outputs are closely matched and human preferences are subjective. We study this failure mode through psychological depth in short stories. Seven readers and an LLM-judge ensemble selected on an earlier scalar PDS dataset evaluated 60 prompt-matched pairs from GPT-5 versus GPT-4o and DeepSeek-R1 versus DeepSeek-V3. Human preferences varied across model families, dimensions, and readers: GPT-5 was preferred overall, whereas the DeepSeek comparison was inconclusive overall and favored V3 on engagement. Across the five criterion-matched PDS dimensions, reasoning outputs won 253 of 272 decisive evaluator comparisons (93.0\%); 28 additional comparisons were exact score ties. Reasoning outputs received 1,219 of 2,100 completed human PDS votes (58.0\%). These different units form a descriptive contrast, not a direct alignment estimate. Five evaluator configurations showed the same directional skew. Group agreement was very low ($\alpha=0.070$), while exploratory within-reader analyses suggested recurring criterion-alignment patterns. Judge scores were also associated with surface features, especially sentence length and lexical diversity. In this setting, an evaluator selected on older scalar annotations produced a much more uniform preference pattern than human readers.
\end{abstract}


==> content_workshop/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Reliable evaluation is foundational to model development: automatic judges are deployed to select checkpoints, compare systems, and provide training signals. LLM-as-a-Judge methods make evaluation scalable, but their validity is not intrinsic and need to be studied closely. Pairwise judging can align with human preference yet amplify evaluator biases \citep{zheng2023judgingllmasajudgemtbenchchatbot,liu2024aligning,jeong-etal-2025-comparative}. Prior work documents position, verbosity, self-preference, inconsistency, and unfairness \citep{li-etal-2025-generation,10.5555/3737916.3740113,stureborg2024large,wang2024large}; less is known about whether judges preserve human heterogeneity in subjective creative evaluation.

Reasoning-enhanced models are typically assessed on mathematical, coding, and factual benchmarks \citep{openai-o1,snell2024scaling,chen2026learning,li202512surveyreasoning,zeng2025thinkingloudreasoningmodels,yu2025benchmarking,10.1145/3774896}, leaving their behavior on creative tasks comparatively understudied. Creative-text evaluation is itself difficult: established fluency-centered metrics can miss literary qualities, and apparent creativity may reflect surface imitation \citep{gomez-rodriguez-williams-2023-confederacy,lu2025rethinking,chakrabarty2024art}. Moreover, disagreement in subjective annotation can encode task ambiguity and value pluralism rather than only noise \citep{clark-etal-2021-thats,sandri-etal-2023-dont,kirk2024prism}. These concerns motivate evaluating both aggregate preference and its distribution across readers.

We examine this question using the Psychological Depth Scale (PDS), which evaluates authenticity, empathy, engagement, emotion provocation, and narrative complexity in fiction \citep{harelcanada2024measuringpsychologicaldepthlanguage}. The setting is deliberately difficult: prompt-matched stories come from frontier model families whose outputs are often close in quality. We compare GPT-5 with GPT-4o under two GPT-5 reasoning-effort settings and DeepSeek-R1 with DeepSeek-V3. These are ecologically relevant model comparisons, not clean causal ablations of reasoning. GPT-5 and GPT-4o differ on many unobserved axes; DeepSeek provides the closest available post-training anchor, but R1 and V3 also differ beyond a single reasoning toggle. We ask whether humans prefer reasoning-model stories (\textbf{RQ1}), whether preferences are consistent across readers and PDS dimensions (\textbf{RQ2}), and whether automatic PDS judges recover the preference as human annotators (\textbf{RQ3}).

Our results expose a sharp human and judge mismatch. Human preferences depend on model family and PDS dimension, with near-chance group agreement and exploratory recurring within-reader associations. Across five PDS dimensions, reasoning outputs won 253 of 272 decisive evaluator comparisons (93.0\%), with 28 exact score ties; reasoning outputs received 1,219 of 2,100 completed human PDS votes (58.0\%). Evaluator pair decisions and individual human votes remain different units, so this is descriptive rather than a direct alignment statistic. Averaging five uncalibrated routed scores produced 59 of 60 pro-reasoning aggregate-PDS decisions, a distinct target from human overall preference. This skew is shared by five evaluator configurations and is associated with surface properties such as sentence length and lexical diversity. We contribute: (1) an exploratory human comparison of reasoning-oriented and comparison-model stories; (2) a target-aware descriptive comparison of evaluator decisions with human preference patterns; and (3) a distributional analysis showing that a point-estimate judge does not represent heterogeneous reader preferences. These results show that development performance on older scalar annotations is insufficient evidence for deployment validity on closely matched pairwise outputs.


==> content_workshop/02_study_design.tex <==
\section{Study design}
\label{sec:study}

\paragraph{Stories and model comparisons.}
We selected 20 open-ended premises from recent r/WritingPrompts posts and Reedsy. For each premise, we generated three model pairings: DeepSeek-R1 versus DeepSeek-V3, GPT-5 (auto effort) versus GPT-4o, and GPT-5 (high effort) versus GPT-4o. This yielded 120 story presentations in 60 pairs, all reusing the same 20 premises. The retained records do not establish whether the GPT-4o text was reused across the two GPT-5 comparisons, so the number of unique texts is between 100 and 120. Generations targeted 400\textendash600 words. The family prompts shared a system instruction, but the DeepSeek user prompt additionally requested ``rich details and depth,'' a potential confound beyond length compliance. DeepSeek-R1 and V3 share a base lineage and provide our closest available anchor for reasoning-oriented post-training \citep{Guo_2025,liu2024deepseek}, but not a surgical ablation. The GPT comparisons are model-level contrasts \citep{singh2025openaigpt5card,hurst2024gpt}; auto and high are two inference-effort settings of GPT-5. Appendix~\ref{app:generation-details} gives prompts and generation details.

\paragraph{Human evaluation.}
Seven undergraduate readers recruited from English and Psychology departments completed a blinded, randomized pairwise study in Label Studio \citep{LabelStudio}. For every pair, each reader selected a preferred story on the five PDS dimensions and on a separate overall-preference question, yielding $7\times60\times6=2{,}520$ completed judgments. The interface required a choice between A and B and did not offer ties or pair-level confidence ratings. Readers could provide free-text rationales and received \$100. The study was deemed exempt by our Institutional Review Board. We monitored completion time, leave-one-reader-out stability, and a post-study survey; Appendix~\ref{app:human-diagnostics} reports these checks and selected rationales.

\paragraph{Automatic evaluator.}
We built a scalar PDS evaluator rather than directly prompting for pairwise choice. Using the original 97-story PDS dataset, we reserved 20\% for selecting few-shot demonstrations and used the remaining 80\% to evaluate Llama and Qwen configurations \citep{grattafiori2024llama3herdmodels,qwen35blog}. Because this same 80\% split selected the best configuration for each dimension and supplied the reported routed correlation ($\rho=0.646$), we treat it as a development/selection-set estimate rather than independent validation. At inference, each story was scored independently on a scale bounded by 1 and 5; retained outputs include fractional scores. Dimension-level preference followed from the higher routed score. Exact score ties were excluded from evaluator preference-rate denominators and reported separately. Judge aggregate-PDS preference compared the uncalibrated arithmetic mean of the five routed dimension scores and is distinct from the separately elicited human overall-preference question. Appendix~\ref{app:evaluator} gives the equation, selection details, configurations, and ties.

\paragraph{Analysis.}
Human preference intervals come from separate intercept-only logistic generalized linear mixed models for each matchup $\times$ criterion, $\mathrm{logit}\,P(y_{ir}=1)=\beta_0+u_i+v_r$, with crossed random intercepts for premise pair $i$ and reader $r$. The 18 GLMM intervals are pointwise and unadjusted for multiplicity, so we interpret cellwise patterns descriptively. We report Fleiss' $\kappa$ and Krippendorff's $\alpha$ \citep{fleiss1971measuring,krippendorff2011computing} as descriptive summaries; with seven readers, reader-level clustering analyses are exploratory. To probe surface associations, we measured word and sentence counts, sentence-length moments, moving-average type-token ratio, MTLD, and story perplexity. Full statistical and surface-feature results appear in Appendices~\ref{app:glmm} and~\ref{app:surface}.


==> content_workshop/03_results.tex <==
\section{Results}
\label{sec:results}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/workshop_results_compact.pdf}
    \caption{Human preferences vary by model pairing and criterion, whereas automatic PDS scoring consistently favors reasoning-oriented outputs. \textbf{(a)} Human preference estimates and pointwise 95\% GLMM intervals; the dashed line marks chance. \textbf{(b)} Decisive reasoning-output wins and exact score ties pooled over all 60 pairs. Percentages report reasoning wins among non-tied evaluator comparisons; comparison-model wins are omitted. Aggregate PDS is distinct from human overall preference, and the panels are a descriptive contrast rather than direct agreement.}
  \label{fig:compact-results}
\end{figure}

\paragraph{Human preference depends on family and dimension.}
Figure~\ref{fig:compact-results}a shows no single pattern across comparisons. Humans preferred GPT-5 overall under auto effort (60.0\%, 95\% CI [52.6, 69.5]) and high effort (62.9\%, [55.9, 72.7]). DeepSeek-R1 trailed V3 overall (42.9\%, [33.7, 50.9]), although this interval includes 50\%. Effects also differed by construct: R1 was disfavored on engagement (39.3\%, [29.6, 46.6]) but favored on emotion provocation (61.4\%, [53.6, 69.9]) and narrative complexity (58.6\%, [50.9, 67.7]). Pooled reader-level reasoning preferences ranged from 36.7\% to 80.0\%. The pooled 55.2\% of 420 overall-preference votes masks model-family and reader-level variation on that question; it neither summarizes the five PDS dimensions nor estimates a universal or causal reasoning effect (Appendix~\ref{app:glmm}).

\paragraph{Group agreement is low; reader structure is exploratory.}
Mean Krippendorff's $\alpha$ was 0.070 and raw agreement was 53.8\%, with weak agreement in every matchup (Appendix~\ref{app:reader-heterogeneity}). The original PDS study reported $\alpha\approx0.72$, but its scalar protocol and different items preclude direct comparison. Low agreement here may reflect limited discrimination, near-indifference, reader subjectivity, or noise. Quality checks reduce but do not eliminate annotation-failure concerns: median time was 108\textendash418 seconds, pacing was stable, and removing any reader shifted rates by only 2\textendash4 points. Exploratory regressions, dimension-to-overall $\kappa$, and rationales suggested recurring criterion-weighting patterns and trade-offs, but seven readers preclude definitive clusters (Appendix~\ref{app:human-diagnostics}).

\paragraph{Automatic PDS scoring strongly favors reasoning outputs.}
Across the five criterion-matched dimensions, reasoning outputs won 253 of 272 non-tied evaluator comparisons (93.0\%; Figure~\ref{fig:compact-results}b), with 28 ties, versus 1,219 of 2,100 human PDS judgments (58.0\%). These pair decisions and individual votes are different units, so the contrast is descriptive rather than direct agreement. The uncalibrated aggregate PDS selected reasoning outputs in 59 of 60 pairs (98.3\%), while humans did so in 232 of 420 separate overall-preference votes (55.2\%); this is also cross-target. Aggregate PDS selected GPT-5 in all 40 GPT-family pairs and R1 in 95.0\% of 20 DeepSeek pairs. Descriptive score advantages were $+0.518$ and $+0.500$ for GPT-5 ($d_z=1.14,1.12$) and $+0.214$ for R1 ($d_z=0.68$). We omit naive paired tests because five dimensions within each pair are dependent. Five configurations' decisive win rates spanned 86.7\% to 98.8\%, so routing alone does not explain the direction (Appendices~\ref{app:evaluator} and~\ref{app:preference-visualizations}).

\paragraph{Surface features are associated with judge scores.}
The difference is not readily interpreted as depth alone. Shorter reasoning-output sentences were associated with human preference ($r=-0.59$; GPT pairs $r=-0.55$), while DeepSeek showed no detectable trend. Judge engagement correlated with mean sentence length at $r=-0.70$, and MATTR correlations were negative across all five dimensions ($-0.37$ to $-0.14$). Reasoning outputs were slightly more lexically uniform but more perplexing to Llama~3.1~70B, arguing against simple familiarity while leaving emotional explicitness and polish as plausible correlates (Appendix~\ref{app:surface}).


==> content_workshop/04_discussion.tex <==
\section{Implications}
\label{sec:implications}

\paragraph{Selection-set performance does not establish transfer.}
The ensemble was more directionally uniform than readers, but the human target and unit changed from scalar ratings to pairwise choices; aggregate PDS also differs from human overall preference. Because the same 80\% split served configuration selection and reported correlation, this is a context-specific warning, not independent evidence of transfer failure. Evaluator reports should document selection, deployment context, calibration, surface sensitivities, and target-matched human checks (Appendices~\ref{app:evaluator} and~\ref{app:surface}), especially when scores gate selection or optimization.

\paragraph{Disagreement should remain visible.}
Near-chance group agreement makes a majority rate incomplete. Preference distributions and reader-level stability expose uncertainty absent from a point estimate (Appendices~\ref{app:reader-heterogeneity} and~\ref{app:human-diagnostics}). This limitation is distinct from the descriptive evaluator-human contrast; subjective-task evaluation should consider target-matched judgment distributions, not only their mean.

\section{Limitations}
This exploratory study uses 20 repeated premises per matchup, one retained generation per condition, seven readers from one university, and one domain. Pairings are noncausal and generation variance is uncontrolled. Forced choice without ties or confidence may turn indifference into preference; fatigue, noise, pluralism, and limited PDS discrimination may contribute to low agreement. The human target changed, $\rho=0.646$ is a selection-set estimate, and surface results are correlational. Broader cohorts, repeated generations, target-matched judges, and out-of-fold validation are needed. The protocol was IRB-exempt; participants consented and were compensated.

\paragraph{Conclusion.}
Humans favored GPT-5 overall but showed no conclusive R1 advantage, while the selected scalar-PDS evaluator was nearly uniformly pro-reasoning on its distinct aggregate target. This exploratory audit motivates target-matched human checks and independent validation before reusing a selected evaluator on a new distribution.
